Rethinking Memory Profiling and Migration for Multi-Tiered Large Memory Systems

Multi-tiered large memory systems call for rethinking of memory profiling and migration because of the unique problems unseen in the traditional memory systems with smaller capacity and fewer tiers. We develop MTM, an application-transparent page management system based on three principles: (1) connecting the control of profiling overhead with the profiling mechanism for high-quality profiling; (2) building a universal page migration policy on the complex multi-tiered memory for high performance; and (3) introducing huge page awareness. We evaluate MTM using common big-data applications with realistic working sets (hundreds of GB to 1 TB). MTM outperforms seven state-of-the-art solutions by up to 42% (17% on average)

==> tables/motivation.tex <==
%The hot pages are those with the number of memory accesses larger than twice in 10s time interval.

\begin{table}[t]
\caption{\textcolor{check}{Number of hot pages identified by various profiling mechanisms in page management systems. Hot pages are accessed at least twice in a profiling interval of 10 seconds.}}
%\vspace{-10pt}
%\small
\footnotesize
\center
\begin{tabular}{|c|c|c|c|}
\hline
             &  Thermostat~\cite{Agarwal:2017:TAP:3037697.3037706} & %AutoNUMA~\cite{autonuma_balance} & 
              AutoTiering~\cite{memory_tiering} & %AutoTiering~\cite{atc21_autotiering} &
              \name \\ \hline \hline
\# hot pages &       90          &       65        %&   65                    &      65           
& 150    \\ \hline

Performance & 2794 s               & 3029  s            %& 11                      & 11                
& 2594 s  \\ \hline
\end{tabular}
\label{tab:prof_limitation}
\end{table}

==> tables/profiling.tex <==
\begin{table}[]
\caption{Comparison between profiling methods in terms of number of PTE walks and overhead.} 
%\vspace{-5pt}
\label{tab:profiling_methods}
\centering
\begin{tabular}{l|l|l|l|l}
\hline
    \# of PTE walks                        & 1s & 2s & 5s & 10s \\ \hline
Application Instrumentation &  1.5K  & 3K   &  8K  &  30k   \\ \hline
Hardware counter sampling   &  30K  &  60K  &  145K  &  290K   \\ \hline
PTE access bit scanning     &  1.5M  & 3M   & 7.5M   &  30M   \\ \hline

\end{tabular}
\end{table}

==> text/evaluation.tex <==
\section{Evaluation}
\label{sec:eval}
%\textcolor{check}{We compare \name with eight existing solutions and use two multi-tiered memory systems for evaluation.}
%\textcolor{jie}{Intel Optane DC PIMM
%%applications (descriptions, configurations, memory footprint)}

\begin{comment}
We aim to answer the following questions for evaluation:
\begin{enumerate}[label=(\roman*)]
    \item What performance does \name achieve on large memory systems with various memory latency and bandwidth  (Section~\ref{sec:eval_overall_perf})? 
    \item Does \name outperform the state-of-art page management solutions on a large memory system (Section~\ref{sec:eval_overall_perf})? 
    \item Are adaptive memory profiling,  holistic migration strategy, and adaptive migration mechanism effective (Sections~\ref{sec:eval_profiling} and~\ref{sec:eval_migration})? 
\end{enumerate}
\end{comment}

%\subsection{Experimental Setup}
\textbf{Testbed.} We evaluate \name on a two-socket machine. Each socket has Intel Xeon Gold 6252 CPU (24 cores), 756GB Intel Optane DC PMM and 96GB DRAM. This machine has four memory tiers (see Figure~\ref{fig:multi-tiered-mem}). We also emulate a four-tiered memory system with doubled latency and bandwidth using memhog in Linux. The emulation launched memhog instances in each memory tier to continuously inject memory access traffic. The details of evaluation platforms show in table~\ref{tab:hardware}.
%Memhog is an artificial memory-intensive workload in Linux used in prior studies to emulate HM~\cite{pact15,Yan:2019:NPM:3297858.3304024}.
%Table~\ref{tab:hardware} summarizes the two platforms. 
Unless indicated otherwise, % Optane uses App Direct Mode, which allows software-based page management, and
we report results on the Optane-based machine (not the emulation platform). 
%\textcolor{jie}{We evaluate \name with setting profiling overhead constrain as 5\% in every profiling interval of 10 seconds.}
%\textcolor{jie}{Unless indicated otherwise, we report results with opt-in mode of transparent hugepages (i.e., madvise), which optimized THP usage and its a setting by default Linux.}
We use \texttt{madvise} for THP~\cite{thp} and uses 2MB as huge page size by default, which    
%page size for contiguous memory allocation. 
is typical in large memory systems. We set the profiling overhead constraint to 5\% and the profiling interval to 10 seconds. This setting is similar to existing works and production environments~\cite{Agarwal:2017:TAP:3037697.3037706, Hirofuchi:2016:RHV:2987550.2987570,meta_tpp, middleware19_profiling}. 
%\textcolor{red}{Jie to add: add a couple of sentences to describe the profiling overhead constraint. See Thermastat as an example. How long is profiling interval}

%{To emulated a multi-tiered memory system we with different memory bandwidth and latency, we inject traffic on machine with Intel Optane DC PMM by memhog. The details of evaluation platforms show in table~\ref{tab:hardware}.}

%\textcolor{jie2}{\textbf{Testbed. }We evaluate \name on machine with Intel Optane DC PMM. To emulated a multi-tiered memory system we with different memory bandwidth and latency, we inject traffic on machine with Intel Optane DC PMM by memhog. The details of evaluation platforms show in table~\ref{tab:hardware}.}

%\textcolor{jie2}{\textbf{Workloads. } We evaluate \name with five big-memory workloads, including one terabyte-level real-world application. The details of workloads show in table~\ref{tab:app_details}. For single-threaded in-memory database VoltDB, We test throughput of one server with eight clients. We evaluate the performance of the remaining multi-threaded workloads with eight physical threads. To eliminate the impact on communication, we deploy server and clients on the same machine for database workload. Note that the memory consumption of each workload is larger than the memory capacity of top-tier memory.}


\textbf{Workloads.} We use large-memory workloads %(in-memory database, graph analysis, and data sorting) 
in Table~\ref{tab:app_details}. Their memory footprints are larger than the fastest two tiers, enabling effectively evaluation on all tiers. Unless indicated otherwise, we use eight application threads per workload.
%{For single-threaded in-memory database VoltDB, We test throughput of one server with eight clients.
%To eliminate the impact on communication, we deploy server and clients on the same machine for database workload. Note that the memory consumption of each workload is larger than the memory capacity of top-tier memory.}

\input tables/hardware_details
\input tables/app_details

\textbf{Baselines.} Eight state-of-the-art solutions are used. %application-agnostic memory management solutions are used for evaluation.
\begin{itemize}[noitemsep]
\item \textit{Hardware-managed memory caching (HMC)} uses the fast memories as hardware-managed cache for slow memories. We use Memory Mode in Optane.
%{In our multi-tiered memory systems, the first two memory tiers (fast memories) are used as the cache for the last two memory tiers (slow memories). In the Optane machine, this is called Memory Mode.}
%\item \textbf{Hardware-managed memory caching}: Optane-based multi-tiered memory system provides Memory Mode, which configures DRAM as hardware-managed DRAM caches for PM. The data migration between DRAM and PM follows fully associative caching algorithm.


\item \textit{First-touch NUMA} is a common allocation policy. It allocates pages in a memory tier close to the running task that first touches the pages. It does not migrate pages. %after memory allocation.% and does not track page hotness.

%\item \textbf{First-touch NUMA}: first-touch NUMA is the default NUMA allocation policy provided by OSes. We use Optane DC PM \textit{APP direct mode} and configure PM as fake NUMA nodes. First-touch NUMA places pages in memory tier until it get full with the following order: local DRAM, local PM, remote DRAM, remote PM. First-touch NUMA policy does not migrate pages after memory allocation.

%\item \textcolor{jie}{Tiered-AutoNUMA~\cite{tiered-autonuma} is a well-established solution to support multi-tired memory systems in Linux. }

\item \textcolor{dong}{\textit{Tiered-AutoNUMA}~\cite{tiered-autonuma} in Linux and \textit{AutoTiering}~\cite{atc21_autotiering}.}

%%%\item \textit{AutoNUMA}~\cite{autonuma} is a well-established solution in Linux. 
%It can reduce memory traffic between NUMA nodes by moving pages close to the running task. AutoNUMA periodically samples limited memory pages (i.e., 256MB memory pages) and does not consider page hotness.

%\item \textbf{AutoNUMA~\cite{autonuma}}: AutoNUMA by is a page migration solution in Linux providing automatic achieving NUMA balancing. AutoNUMA periodically samples memory chunks to identify cross NUMA accesses, and migrates the pages to the NUMA node where the task is running. AutoNUMA only balances page accesses between local and remote nodes but does not balance page accesses between DRAM and PM nodes.

%\item \textcolor{check}{\textit{Memory optimizer~\cite{intel_mem_optimizer}} is an industry-quality solution from Intel for two-tiered heterogeneous memory. It randomly samples pages for profiling and migrates pages between two memory tiers within the same socket, but not across sockets.}

%\item \textit{Memory-optimizer~\cite{intel_mem_optimizer}} is a solution from Intel.


%We configure PM as fake NUMA nodes to use Memory-optimizer from Intel. Memory optimizer treats the system as two CPU sockets, and each CPU socket contains one DRAM and one PM. Memory optimizer provides page migration between DRAM and PM within the same CPU socket. There is no page migration between two CPU sockets.

%\item \textbf{Memory-optimizer~\cite{intel_mem_optimizer}}: We configure PM as fake NUMA nodes to use Memory-optimizer from Intel. Memory optimizer treats the system as two CPU sockets, and each CPU socket contains one DRAM and one PM. Memory optimizer provides page migration between DRAM and PM within the same CPU socket. There is no page migration between two CPU sockets.


%%%\item \textit{Memory-tiering}~\cite{memory_tiering} is from Intel and extends AutoNUMA.
%%from Intel, extends AutoNUMA, and uses uncontrolled random-page profiling.
%{It allows page migration within and across sockets. But it randomly samples limited memory pages and promotes hot pages slowly across memory tiers.}

%We configure PM as fake NUMA nodes to use Intel Memory-tiering. Similar as Memory-optimizer, Memory-tiering views Optane-based multi-tiered memory system as two CPU sockets. And each CPU socket contains one DRAM and one PM. Memory-tiering provides page migrating between CPU sockets and within the same CPU socket.

%\item \textbf{Memory-tiering~\cite{memory_tiering}}: We configure PM as fake NUMA nodes to use Intel Memory-tiering. Similar as Memory-optimizer, Memory-tiering views Optane-based multi-tiered memory system as two CPU sockets. And each CPU socket contains one DRAM and one PM. Memory-tiering provides page migrating between CPU sockets and within the same CPU socket.

%%%%\item \textit{AutoTiering}~\cite{atc21_autotiering} extends NUMA balancing~\cite{autonuma_balance} for multi-tiered memory. %%%%We enable its opportunistic promotion/migration and background demotion for high performance.

%It is based on AutoNUMA, and introduces flexible page migration between memory tiers. However, it does not have a systematic migration strategy guided by page hotness, and uses random sampling as AutoNUMA. 
%\textcolor{jie2}{We enable opportunistic promotion and migration (OPM) and background demotion in AutoTiering during the evaluation, which shows the best performance in~\cite{atc21_autotiering}. } 
%\item \textbf{AutoTiering~\cite{atc21_autotiering}}: AutoTiering is based on AutoNUMA, which proposes opportunistic promotion and migration between DRAM and PM nodes. Specifically, AutoTiering 
%\item \textcolor{jie}{\textit{HeMem}~\cite{sosp21_hemem} is a state-of-the-art solution for two-tierd PM-based HM. HeMem leverages PEBS-based scanning to find hot pages and promotes hot page to fast memory tier.}
\item \textit{HeMem}~\cite{sosp21_hemem} is for two-tiered systems. HeMem leverages performance counters alone to find hot pages. %%%and promotes hot page to the fast memory tier.

\item \textit{Thermostat}~\cite{Agarwal:2017:TAP:3037697.3037706} is for two-tiered systems. It allocates all pages in the fast tier and selectively moves them to the slow tier. It cannot support applications with footprint larger than the fast tier. Thus, we do not evaluate its page migration but only evaluate its profiling method. 

%It randomly samples pages for profiling. 

\item \textit{DAMON}~\cite{middleware19_profiling, damon} is a Linux profiling tool at the memory region granularity. We use it to evaluate profiling quality.

\item \textit{Nimble}~\cite{Yan:2019:NPM:3297858.3304024} is a page migration mechanism using bi-direction page copy and parallel page copy. \name includes the techniques in Nimble but adds adaptive migration. We use Nimble to evaluate our page migration mechanism.

\end{itemize}




\subsection{Overall Performance}
\label{sec:eval_overall_perf}
%baseline intel tiered memory(AutoNUMA balancing), Memory mode, NUMA first touch.
%(1) breakdown application execution time and data migration time
%2) traffic 
%(3) inject latency \& bandwidth to simulate different big mem system

\begin{figure}[tb]
\centering
\includegraphics[width=0.9\columnwidth]{figures/overall_perform.pdf}
\vspace{-10pt}
\caption{Overall performance (normalized to \textcolor{dong}{first-touch NUMA}'s) using existing solutions and \name on Optane.} 
\label{fig:overall_optane}
\end{figure}
%\textcolor{jie}{Execution time of using hardware-managed memory caches (HMC), First-touch NUMA, AutoNUMA, Memory-optimizer, Memory-tiering, AutoTiering and \name on Optane-based multi-tiered memory system.}


\textbf{Optane-based multi-tiered system.}
Figure~\ref{fig:overall_optane} shows that \name outperforms all baselines. %including stock Linux kernel, industry-quality solution from Intel, and state-of-the-art multi-tiered memory management solution. 
We have five observations. 

%HMC performs poorly with memory-consuming workloads. 
(1) \name outperforms HMC by up to 40\% (avg. 19\%). HMC incurs write amplification when cache misses occur~\cite{9408179}, causing unnecessary data movement and low performance.
%(1) Hardware-managed memory caching (HMC) performs poorly with memory-consuming workloads which have hundreds of gigabyte memory consumption. \name outperforms HMC by 55\% on average. Using fast memories as cache incurs write amplification in big memory system when cache miss happens frequently.

%(2) First-touch NUMA statically places pages near to CPU during the page allocation.  First-touch NUMA performs better than HMC and AutoNUMA in some workloads, which indicates page migration does not always help performance improvement. Without knowing the overall page access information, unnecessary page migration can cause large performance overhead. \name outperforms first-touch NUMA in all cases, and gains up to 45\% performance improvement. 

(2) \name outperforms first-touch NUMA by up to 24\% (avg. 17\%). Without page migration, first-touch NUMA outperforms HMC on VoltDB and BFS, and outperforms tiered-AutoNUMA on Cassandra and BFS, indicating that page migration is not always helpful. HMC performs worse because of unnecessary page movement. tiered-AutoNUMA has worse performance because it cannot effectively identify hot pages. %\name does not have those problems. 

%(3) \name outperforms AutoNUMA up to 52\%. AutoNUMA in Linux is capable of transparently migrating frequently accessed data pages between NUMA nodes. Specifically, AutoNUMA is designed to balance the memory access between two sockets, but does not support page migration between different memory tiers within the same socket. Figure~\ref{fig:overall_optane} reveals that using AutoNUMA fail to take full advantage of all memory tiers in big memory system.

%%%%%%%%%%(3) \name outperforms AutoNUMA by up to 40\% (avg. 19\%). AutoNUMA does not support page migration between memory tiers within the same socket (Memory-tiering, which is an extension to AutoNUMA, supports so), and hence fails to take full advantage of all memory tiers.


(3) \name outperforms tiered-AutoNUMA by up to 37\% (avg. 23\%). Tiered-AutoNUMA provides page migration across all memory tiers. However, tiered-AutoNUMA promotes hot pages slowly, %tier-by-tier, 
which wastes the opportunity to accelerate application execution in fast memory. 

%(4) \name outperforms Memory-tiering by up to 45\% (avg. 22\%). Different from AutoNUMA and Memory-optimizer, Memory-tiering enables page migration across all memory tiers. However, it promotes hot pages tier by tier instead of using fast promotion as \name, delaying the opportunity to improve performance using the fastest memory.


(4) \name outperforms AutoTiering by up to 42\% (avg. 17\%). AutoTiering uses random sampling and opportunistic demotion, failing to effectively identify pages for migration.

(5) \name outperforms the solution of disabling performance counter for profiling (MTM-w/o-PEBS in the figure) by up to 10.6\%.  %(avg. 5.4\%). 
Lack of efficient methods to detect hot regions in the slowest memory tier, MTM-w/o-PEBS fails to provide high quality profiling result to guide page placement.
% Memory-optimizer by up to 65\% (avg. 32\%). Lack of page migration across sockets, Memory-optimizer fails to fully leverage the 2nd fastest tier on a socket for the application on the other socket.
%(6) \name outperforms AutoTiering up to 35\% and by 15\% on average for all evaluated workloads. AutoTiering explores all memory tiers in multi-tiered memory system based on periodically profiling the hotness of random memory chuck. Furthermore, AutoTiering opportunistically demotes pages from the upper-tier memory to other memory tiers to create free space. During the lack of global view of pages hotness with random sampling, AutoTiering can not beat performance of \name in all evaluated workloads.


%%%\textcolor{red}{Jie TODO: "In Figure 5, first-touch NUMA is often second-best after Titan. I would love to see some discussion of why this is the case, since it does nothing sophisticated, while Optane's hardware cache and the MO/MT setups actually try to actively improve things, yet seem to make them worse. To me, this was an unexpected result that I'd like to see discussed in more detail."}


%\textbf{Emulated multi-tiered memory system.} We further test the performance of  and \name on the emulated multi-tiered memory system. We inject latency on each memory tier in Optane-based machine and increase the latency different between each memory tier. Table~\ref{tab:hardware} shows the details of the system. We do not evaluate hardware-managed memory caching (HMC) in emulated multi-tier memory system because we can not inject latency in fast memories when we enable HMC. As shown in figure~\ref{fig:perform_emulated}, \name maintains the same performance trend as that on Optane-based multi-tiered memory system: \name outperforms First-touch NUMA, AutoNUMA, Memory-optimizer, Memory-tiering, AutoTiering by 19\%, 38\%, 20\%, 26\%, 17\% on average with five big memory workloads.


\textbf{Emulated multi-tiered memory system.} Figure~\ref{fig:perform_emulated} shows that on the emulated platform, \name maintains the same performance trend as on the Optane-based testbed -- it outperforms first-touch NUMA, tiered-AutoNUMA, AutoTiering and MTM-w/o-PEBS by 19\%, 26\%, 17\%, and 14\% respectively. Note that HMC is not evaluated because when HMC is used, fast memory tiers are hidden from software and we cannot inject latency into fast memory. 
\begin{figure}[t!]
    \centering
        \includegraphics[width=0.9\columnwidth]{figures/perform_emulated.pdf}
        \vspace{-10pt}
        \caption{Performance comparison between existing solutions and \name on the emulated multi-tiered memory system. The performance is normalized by First-touch NUMA performance.}
        \label{fig:perform_emulated}
\end{figure}

\textbf{Performance breakdown.}
We show the breakdown into application execution time, migration time, and profiling time in Figure~\ref{fig:perform_breakdown}. The migration time is the overhead exposed on critical path, excluding asynchronous page copying time. We only compare tiered-AutoNUMA, MTM-w/o-PEBS and \name because they are the only solutions that can leverage all four memory tiers for migration. We add first-touch NUMA as a performance baseline because evaluated solutions use first-touch NUMA for memory allocation. In all cases, the profiling overhead falls within the profiling overhead constraint.

%We study the profiling and migration overhead for Memory-tiering, AutoTiering and \name, which provide profiling and page migration for all memory tiers on multi-tiered memory systems. We add First-touch NUMA result into comparison since Memory-tiering, AutoTiering and \name use the first-touch policy as memory allocation policy. Specifically, we measure the time spend on profiling, and migration in different memory management solution separately. Figure~\ref{fig:perform_breakdown} shows the result. We have the following observations.

%(1) Comparing with First-touch NUMA, Memory-iering, AutoTiering and \name have less application execution time by 13\%, 14\% and 24\% on average respectively. However, for Memory-iering and AutoTiering, the application execution time reduction is less than or equal to the overhead brought by profiling and migration in some workloads. Therefore, the performance of Memory-iering and AutoTiering is no better than the first-touch memory allocation policy without page migration in some cases.

With tiered-AutoNUMA, the time reduction is lower or equal to the overhead of profiling and migration (see VoltDB and Cassandra). Hence, they perform worse than first-touch NUMA without page migration. Compared to tiered-AutoNUMA, \name spends similar time in profiling but 3.5$\times$ faster in migration, reducing the execution time by 21\% on average. Compared to AutoTiering, \name spends similar time in profiling but 25\% faster in migration, and reduces the execution time by 19\% on average. %Because of the effectiveness of page sampling and migration, \name obtains better performance.  

\textbf{Evaluation of performance-counter assistance.} MTM-w/o-PEBS in Figure~\ref{fig:perform_breakdown} does not use performance counters to guide profiling. It performs worse than \name because PEBS improves profiling quality. For GUPS, it performs 10.6\% worse. The overhead of PEBS is less than 1\% in all cases.
%\textcolor{jie}{MTM-w/o-PEBS in Figure~\ref{fig:perform_breakdown} does not use performance counters. It performs 10.6\% worse than \name with GUPS, and 5.6\% on average, because PEBS improves the profiling quality without increase profiling overhead. Specifically, the difference of profiling and migration overhead for \name and MTM-w/o-PEBS is less than 1\% in all evaluated workloads. Meanwhile, the application execution time is \name outperforms MTM-w/o-PEBS by 10.4\% in GUPS, which indicates that PEBS is helpful to capture hot memory regions more accurately. } 



%(2) Compared with Memory-tiering, \name spends only 69\% more time on profiling and 3.5x less time on migration. \name also reduces the application execution time by 11\% comparing with Memory-tiering. Because of the effectiveness of page sampling, migration strategy, and migration mechanism, \name obtains more performance gains in page migration than Memory-tiering does.  

%(3) Compared with AutoTiering, \name spends 69\% more time on profiling, 1.25x less time on migration. \name also reduces the application execution time by 5\% comparing with AutoTiering. Figure~\ref{fig:perform_breakdown} reveals that with adaptive page sampling, \name provides more accurate memory profiling result, and can effectively guide page migration.



\begin{figure*}[t!]
    \centering
        \includegraphics[width=2\columnwidth]{figures/perform_breakdown.pdf}
        \vspace{-5pt}
        \caption {Breakdown of application execution time. Each bar is normalized by the execution time of first-touch NUMA.}
        \vspace{-5pt}
        \label{fig:perform_breakdown}
\end{figure*}

%\textbf{Number of memory accesses.} We further compare the number of memory accesses from application in each memory tier of \name and that of Memory-tiering with voltDB. %Table~\ref{tab:traffic} shows the result. To measure the number of memory accesses comes from application only, we first count number of memory accesses happen in each memory tier by using system monitor~\cite{intel_pcm}. We also intercept migration call in Memory-tiering and \name during the execution, which can be used to analyze the number of memory accesses incurred by page migration. Such that we can get the number of memory accesses happen due to application execution instead of page migration. 

\textbf{Number of memory accesses.} We count the number of memory accesses in each memory tier when running VoltDB. %\textcolor{jie}{For single-threaded in-memory database VoltDB, We test throughput of one server with eight clients. To eliminate the impact on communication, we deploy server and clients on the same machine with different processor.}
We only report the results for tiered-AutoNUMA, MTM-w/o-PEBS, and \name because only they can leverage all four memory tiers for migration. We use Intel Processor Counter Monitor~\cite{intel_pcm} to count the number of memory accesses and exclude memory accesses caused by page migration. This counting method allows us to evaluate the number of memory accesses from the application (not from page migration). Table~\ref{tab:traffic} shows the results \textcolor{dong}{where there are eight VoltDB clients residing in one processor, and the view of tiered memory is defined from their view.} Table~\ref{tab:traffic} shows that with \name, the number of memory accesses in the fastest memory tier (tier 1) is 20\% and 14\% more than with tiered-AutoNUMA and AutoTiering. This indicates that \name effectively migrates frequently accessed pages to the fast tier for high performance.

%\textbf{Number of memory accesses.} We count the number of memory accesses at each memory tier when running GUPS. We report the results for Memory-tiering, AutoTiering, MTM-w/o-PEBS and \name, because they are the only solutions that leverage all memory tiers for migration. Table~\ref{tab:traffic} shows the results. We use Intel Processor Counter Monitor~\cite{intel_pcm} to count the number of memory accesses and then exclude memory accesses caused by page migration. This counting method allows us to evaluate how many memory accesses from the application (not from page migration) happen on memories. 

%Table~\ref{tab:traffic} shows that using \name, the number of memory accesses happen in top-tier is 20\% more that that of using Memory-tiering. This indicates \name effectively migrate more frequent accessed pages into top-tier memory.



\input tables/traffic

\begin{comment}
\begin{figure}[t!]
    \centering
        \includegraphics[width=1\columnwidth]{figures/time_serial_heatmap.pdf}
        \caption {Number of memory regions using \name with GUPS.}
        \label{fig:time_serial_heatmap}
\end{figure}
\end{comment}

\input tables/mem_regions

\textbf{Statistics of memory regions.} On average, the number of memory regions merged and split in a profiling interval is 3.4\% of all memory regions, as reported in Table~\ref{tab:mem_regions}. Compared with DAMON, \name has less merging/splitting because of performance counter guidance and effective formation of memory regions. For example, GUPS with \name has 12\% less merging and 32\% less splitting than with DAMON.

%\textcolor{jie}{Table~\ref{tab:mem_regions} shows the results for \name. \name manages over one thousands memory regions for large-memory workload. Typically, memory region merge and split do not happen very often. On average, the number of memory regions which are merged and split in a profiling interval is 3.4\% of the total number of memory region managed by \name for all six applications. In general, compared with DAMON, \name has less merge/split operations and less memory regions. For example, for GPUS, the average number of merged and split memory regions in a profiling interval in \name are less than that of DAMON by 12\% and 32\%, respectively.}


%\textcolor{jie}{\name dynamically split and merge memory regions based on detecting memory access temporal and spatial locality. Figure~\ref{fig:time_serial_heatmap} shows total number of memory regions, and the number of memory region merged and splited in each profiling interval when we execute GUPS with \name. At the beginning execution of GUPS, \name splits the memory space used in GUPS into 512 memory regions. In each profiling interval, \name splits and merges less than 50 memory regions. The total number of memory regions tracked by \name keep reducing. }



\textbf{Scalability of \name}. We evaluate the scalability of \name with VoltDB by increasing  the number of clients. We see the memory consumption increases from 300GB to 1.2TB. We compare the performance of \name, HMC, first-touch NUMA, and AutoTiering. %\textcolor{red}{HMC and first-touch NUMA do not require any helper thread for memory management}. 
We evaluate AutoTiering since it has the second-best performance among all we evaluate. %\textcolor{red}{AutoTeiring and \name use helper threads for profiling and migration.}
%and they use hyperthreads for \textcolor{dong}{profiling and migration} \textcolor{red}{when no physical thread is available}. 
Figure~\ref{fig:scalibility} shows that \name consistently outperforms HMC, first-touch NUMA, and AutoTiering by 19\%, 10\%, and 8\% on average.  %as the number of application threads increases.
\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/scalibility.pdf}
    \vspace{-10pt}
  \caption{Execution time of VoltDB with different number of client threads.}\label{fig:scalibility}
  \vspace{-10pt}
\end{figure}

\begin{comment}
\begin{figure*}[!htb]
\minipage{0.32\textwidth}
  \includegraphics[width=\linewidth]{figures/scalibility.pdf}
  \caption{Execution time of VoltDB with different number of client threads.}\label{fig:scalibility}
\endminipage\hfill
\minipage{0.32\textwidth}
  \includegraphics[width=\linewidth]{figures/THP_new.pdf}\caption{SSSP with \name and different THP configurations.}
    \label{fig:thp}
\endminipage\hfill
\minipage{0.32\textwidth}%
  \includegraphics[width=0.8\linewidth]{figures/hemem_res.pdf}
        \caption{Evaluation of \name on two-tiered HM and comparison with HeMem.}
        \label{fig:hemem}
\endminipage
\end{figure*}
\end{comment}

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/THP.pdf}\caption{SSSP with \name and different THP configurations.}
    \label{fig:thp}
\end{figure}




\begin{comment}
\begin{figure*}[!htb]
\minipage{0.6\textwidth}%
  \includegraphics[width=0.9\linewidth]{figures/test.pdf}
      \vspace{-5pt}
        \caption{The heatmap of memory accesses in GUPS using (a) DAMON and (b) \name under the same profiling overhead (5\%).}
        \label{fig:heatmap}
\endminipage\hfill
\minipage{0.4\textwidth}
    \includegraphics[width=0.9\columnwidth]{figures/profiling.pdf}
        \vspace{-10pt}
        \caption{Evaluation of the effectiveness of adaptive memory regions (``AMR''), adaptive page sampling (``APS''), and profiling overhead control (``OC'') using VoltDB.}
        \label{fig:profiling}
\endminipage
\end{figure*}
\end{comment}



\begin{comment}
\begin{figure}[t!]
    \centering
        \includegraphics[width=.9\columnwidth]{figures/scalibility.pdf}
        %\vspace{-10pt}
        \caption{Execution time of VoltDB with different number of client threads.}
        \label{fig:scalibility}
\end{figure}
\end{comment}
%\textcolor{jie}{\textbf{Working with transparent huge pages (THP).} We evaluated \name and all baselines with THP enabled on optane-based multi-tiered memory system. We test sssp, which is one of the largest memory applications we evaluated, with 2MB and 1GB huge pages. Figure~\ref{fig:thp} shows the result. We enable THP at system-wise.}

\textbf{Evaluation with different THP settings.} Figure~\ref{fig:thp} shows the results using \texttt{madvise} and \texttt{always} as THP setting. We evaluate SSSP, because it has the largest memory consumption among all evaluated applications. The results confirm that \name consistently outperforms other solutions. %even at different huge page sizes.

\begin{comment}
\begin{figure}[t!]
    \centering
        \includegraphics[width=0.9\columnwidth]{figures/THP.pdf}
        %\vspace{-10pt}
        \caption{\textcolor{jie}{Evaluating \name with different large page sizes. We use the SSSP application for evaluation.}}
        \label{fig:thp}
\end{figure}
\end{comment}
%\textcolor{jie}{\textbf{Working on two-tiered HM.} We compare \name with HeMem using a single socket with the 1st tier and 3rd tier on our evaluation platform.}

%\begin{comment}
\textbf{Evaluation on two-tiered HM and comparison with HeMem.} 
%We compare \name with HeMem~\cite{sosp21_hemem}, a state-of-the-art. 
The evaluation is performed on a single socket with two tiers, using  GUPS~\cite{gups} as in HeMem~\cite{sosp21_hemem}.
%, because GUPS allows us to easily change the working set size to evaluate the effectiveness of HeMem and \name.
Figure~\ref{fig:hemem} reports using 16 and 24 application threads. The results show that when the working set size fits in the fast memory tier (i.e., the ratio in the \texttt{x} axis is smaller than 1.0), \name performs similarly to HeMem at 16 threads but better at 24 threads. Once the working set size exceeds the fast memory, HeMem fails to sustain performance at 24 threads while \name still sustains higher performance at 24 threads than 16 threads. \name performs better because its profiling method can quickly adapt to changes in memory accesses and identify more hot pages.
%or better than HeMem, because of smaller profiling overhead (); when
%\name disables profiling when the working set size is smaller than the fastest memory size

%\begin{comment}
\begin{figure}[t!]
    \centering
        \includegraphics[width=0.9\columnwidth]{figures/hemem_res.pdf}
        \vspace{-10pt}
        \caption{Evaluation of \name on two-tiered HM and comparison with HeMem.}
         \vspace{-10pt}
        \label{fig:hemem}
\end{figure}
\begin{comment}

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/hemem_res.pdf}
    \vspace{-15pt}
        \caption{Evaluation of \name on two-tiered HM and comparison with HeMem.}
        \label{fig:hemem}
\end{figure}

\end{comment}
%When the ratio of working set size to the fast memory size is larger than 1.5, HeMem cannot run.
%\end{comment}
\subsection{Effectiveness of Adaptive Profiling}
\label{sec:eval_profiling}
%To demonstrate the effectiveness of adaptive profiling method in \name, we compare profiling quality and overhead of \name with two state-of-the-art sampling-based profiling methods, which are profiling method used in Memory-tiering~\cite{memory_tiering} and in Thermostat~\cite{thermostat_asplos17}. We do not compare profiling method in \name with AutoNUMA and AutoTiering because both of them use the same random sampling method as Memory-tiering to identity hot pages. 

\textbf{Comparison with tiered-AutoNUMA and Thermostat.} We study profiling quality and overhead, and compare \name with two sampling-based profiling methods: one used in tiered-AutoNUMA and AutoTiering, and the other used in Thermostat. We use tiered-AutoNUMA and Thermostat, and replace their migration with \name's,  which excludes the impact of migration on performance, and is fair.

%Memory-tiering random samples a fixed-size memory chunk without considering temporal or spatial locality. Specifically, Memory-tiering scans every 4KB page PTE access bit in a sampled virtual space in each profiling interval. The sampled virtual space are randomly selected every two profiling intervals. 

%Thermostat selects one 4KB page in every 2MB memory region as the representative for memory region. Thermostat tracks every representative by poisoning PTE reserved bit and counting the number of protection fault. Comparing with scanning PTE access bit used in \name and Memory-tiering, poisoning PTE reserved bit and counting protection fault in page bring more accurate access information but larger profiling overhead. 

The profiling method in tiered-AutoNUMA randomly chooses a 256MB virtual address space in each profiling interval, and then manipulates the present bit in each PTE in the chosen address space. This method tracks page accesses by counting page faults. The profiling method in Thermostat randomly chooses a 4KB page out of each 2MB memory region for profiling. This method manipulates page protection bits in PTE and leverages protection faults to count accesses.

%To evaluate the effectiveness and overhead of profiling methods in Memory-tiering, Thermostat and \name, we evaluate the end-to-end performance by using the same migration strategies and the same migration mechanism based on profiling results come from different profiling methods. Specifically, we set profiling interval length as 5s for each profiling method. Each profiling method have different profiling overhead. Figure~\ref{fig:profling} shows the result. \name outperforms the system using profiling methods in Memory-tiering and Thermostat by 17\% and 7\% .


%To evaluate the effectiveness and overhead of profiling methods in Memory-tiering, Thermostat and \name, we evaluate the end-to-end performance by using the same migration strategies and the same migration mechanism based on profiling results come from different profiling methods. Specifically, we set profiling interval length as 5s for each profiling method. Each profiling method have different profiling overhead. 

%Figure~\ref{fig:profling} shows the result. \name outperforms the system using profiling methods in Memory-tiering and Thermostat by 17\% and 7\% .

%We observe that Thermostat has higher profiling overhead than profiling methods in Memory-tiering and \name by 6x and 2.5x, respectively, since poisoning PTE reserved bit and counting protection fault is more expensive compared with scaning PTE. Furthermore, the profiling overhead can not be bounded since the representative of memory region can be accessed multiple times in one profiling interval, which leads to frequent protection fault happening and further increases the profiling overhead.     

%Figure~\ref{fig:profling} also shows that with Memory-tiering, the application execution time is longer than with Thermostat and \name by 24\% and 22\% respectively. This indicates that profiling with random samples can not provide useful hits used in page migration. 

%The adaptive profiling in \name \textcolor{red}{carefully selects} samples in memory region by considering temporal and spatial locality. Helping with overhead control, \name achieves good balance between profiling quality and profiling overhead.

Figure~\ref{fig:profiling} shows that \name outperforms tiered-AutoNUMA and Thermostat by 17\% and 7\%, respectively. The profiling overhead in Thermostat is 6$\times$ higher than in tiered-AutoNUMA, %has higher profiling overhead than Memory-tiering by 6x 
because the number of sampled pages for profiling in Thermostat is much larger than that in tiered-AutoNUMA. The profiling overhead in Thermostat is 2.5$\times$ higher than in \name, 
%Thermostat has higher profiling overhead than \name by 2.5x, 
because manipulating reserved bits in PTE and counting protection faults in Thermostat is more expensive than scanning PTEs in tiered-AutoNUMA and \name. With tiered-AutoNUMA, the application run time is longer than with \name by 22\%. This indicates that random sampling-based profiling is not as effective as our adaptive profiling. %The adaptive profiling, when choosing samples, considers both temporal and spatial locality, and aims to maximize profiling quality within a profiling overhead constraint, which is missing in random sampling.

\begin{figure}[t!]
    \centering
        \includegraphics[width=\columnwidth]{figures/test.pdf}
        \vspace{-20pt}
        \caption{The heatmap of memory accesses in GUPS using (a) DAMON and (b) \name under the same profiling overhead (5\%).}
        \label{fig:heatmap}
        %\vspace{-5pt}
\end{figure}

%We normalize the memory access frequency in each profiling interval. 


\textbf{Comparison with DAMON.}
We compare DAMON and \name in terms of profiling quality. We use GUPS that randomly accesses 512GB memory with 24 threads. Specifically, 20\% of GPUS' memory footprint is randomly selected as the hotset. Each thread randomly updates the memory 1M times, and 80\% of them happens in the hotset. %The probability for an update to happen in the hotset is 80\%. 
1M-updates repetitively happens, so that there is variance on hot pages. 
%After 1M updates (taking about 50s), GUPS re-selects the hotset so that there is variance on hot pages. 
Using knowledge on GUPS, we know there are three hot data objects:  the indexes to access the hotset (labeled as ``A''), the hotset information (labeled as ``B''), and the hotset (labeled as ``C'').
%\textcolor{jie}{We compare DAMON and \name in terms of profiling quality. We use GUPS that  with executing Giga-updates per second (GUPS). We set GUPS randomly access 512GB memory with 24 threads. Specifically, GUPS randomly select 20\% of the continues memory as the hotset. Each thread randomly updates the memory 1M times. The probability for each update happens on the hotset is 80\%. After 1M updates ends (takes about 50s in our case), GUPS will re-select the hotset. }


%\textcolor{jie}{We analysis the profiling results by mapping the hot memory regions (i.e., area A, B and C) in figure~\ref{fig:heatmap} with recorded GUPS execution trace. We have following observations: (1) Area A is detected by both DAMON and \name, which is used to store indexes for random access for each thread. Compared with GUPS execution traces, we found both DAMON and \name has false positive pages counted as hot pages, this is because the profiling in DAMON and \name are based on memory region. Additionally, DAMON has much more false positive detected than \name, due to DAMON's random memory region split. (2) Area B is only detected by \name, which is used to store hotset information. Compared with area A, area B has been accessed less frequently.  (3) Random accesses happen in area C. Compared with DAMON, \name can detect relative hot memory regions more efficiently. Compared with DAMON, \name leverages PEBS to have more accurate access tracing hints in slow memory tiers, and saving more profiling budget to profile more accurately in fast memory tiers.}


Figure~\ref{fig:heatmap} shows results. (1) \name finds C, while DAMON cannot because of its slow response. (2) \name finds B, but DAMON cannot because its memory regions are initially set based on the virtual memory area tree, which is too coarse-grained to capture B even after splitting regions. (3) DAMON and \name find A, but the scope of A found by \name is correctly narrowed down, which reduces unneeded migration. %The accurate profiling comes from the effective formation of memory regions.

%We further evaluate the major profiling techniques in \name include: (1) adaptive memory regions, (2) adaptive page sampling and (3) profiling overhead control. To study how above techniques helps \name improve profiling quality and control profiling overhead, we measure the performance breakdown for profiling techniques by disabling each profiling technique. Figure~\ref{fig:profling} shows the result. We have following observations. (1) Without adaptive memory regions, \name does not perform memory regions merging/splitting. Such that the application execution time is 22\% longer compared with enabling adaptive memory regions. The performance loss of disabling adaptive memory regions reveals that the design of adaptive memory regions is critical to improve profiling quality. (2) We disable adaptive page sampling by distributing profiling samples without considering temporal locality, and randomly select memory regions to add more samples in it. Such that the application execution time is 21\% longer compared with enabling adaptive page sampling. The performance loss reveals that the distribution of profiling samples impacts profiling quality. (3) We disable profiling overhead control by setting $\tau_1=\tau_2=0$ during the profiling, which means the memory region merging/splitting will not happen for reducing profiling overhead. We ensure each memory region has at least one samples. The execution time spends on profiling in \name increases by 3x when we disable profiling overhead control.  

%We further evaluate three major profiling techniques (i.e., adaptive memory regions, adaptive page sampling, and profiling overhead control). We disable them one by one and then examine the performance difference. The last three groups of bars in Figure~\ref{fig:profiling} show the evaluation results.

We further evaluate the following profiling techniques and disable them one by one to examine performance difference.

\textbf{Evaluation of adaptive memory regions.} 
%The technique of adaptively merging and spliting memory regions aims to improve profiling quality. 
We disable adaptive memory regions but respect the profiling overhead constraint. Figure~\ref{fig:profiling} shows the application execution time is 22\% longer, although the overhead constraint is met. Such a loss indicates that hot memory regions are not effectively identified without adaptive regions and hence placed in slow memory.


\textbf{Evaluation of adaptive page sampling.} This technique distributes PTE scans between memory regions by using time-consecutive profiling, which includes information on temporal locality. We disable it and randomly distribute PTE scans between memory regions, and observe 21\% performance loss. %in Figure~\ref{fig:profiling}. This indicates the importance of using temporal locality as the metric to guide the selection of samples.

\textbf{Evaluation of profiling overhead control.} We set $\tau_1=\tau_2=0$ (i.e., no merging/splitting memory regions) and observe that the profiling time is increased by 3$\times$ in Figure~\ref{fig:profiling}.

%We disable profiling overhead control by setting $\tau_1=\tau_2=0$ (i.e., no merging/splitting memory regions) and removing the control of the number of page samples ($num\_{ps}$ in Equation~\ref{eq:profiling_overhead_control}). We observe that the profiling time is increased by 3x in Figure~\ref{fig:profiling}.


\begin{figure}[t!]
    \centering
        \includegraphics[width=0.95\columnwidth]{figures/profiling.pdf}
        \vspace{-10pt}
        \caption{Evaluation of the effectiveness of adaptive memory regions (``AMR''), adaptive page sampling (``APS''), and profiling overhead control (``OC'') using VoltDB.}
        \label{fig:profiling}
\end{figure}



%Execution time breakdown for system with profiling methods used in Thermostat, Memory-tiering and profiling technique in \name. ''AMR``, ''APS``, and ''OC`` stands for ''adaptive memory regions``, ''adaptive page sampling`` and ''overhead control`` respectively.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{comment}
\begin{figure}[t!]
    \centering
        \includegraphics[width=\columnwidth]{figures/profiling_overhead.pdf}
        \caption{Execution time with setting various of profiling overhead targets when execute voltDB with \name. }
        \label{fig:overhead}
\end{figure}

We further study the relation between profiling overhead and profiling quality. Figure~\ref{fig:overhead} shows the result. We set profiling interval length as 5s and test a set of profiling overhead targets. As the profiling target increase from 1\% to 10\%, the application execution time decrease by 12\%, which reveals that the profiling quality can be improved by increasing the number of samples in profiling. 
However, better profiling quality does leads to better system performance, since the performance benefit from more accurate profiling result may not able to cover extra profiling overhead we have to pay. As shown in figure~\ref{fig:overhead}, the end-to-end performance decreases by 7\% as the profiling target increase from 5\% to 10\%.  
%\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Thermostat does not have (1)-(4); has spatial locality 
%Intel mem tiering does not have (1) -(4)
%Intel mem optimization does not have (1)-(4)

%Distinguishing points:
%Capturing both temporal and spatial locality; (2) more accurate profiling

%\textcolor{jie2}{Thermostat~\cite{thermostat_asplos17} profiles every 2MB huge page access by tracking one of the representative 4KB page.  }


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{comment}
\subsection{Effectiveness of Migration Strategy}
\label{sec:eval_migration}
%(1) hierarchical mode vs. our mode
%(2) Number of migration;
%(3) migrated data size;
%\name adopts ``fast promotion but slow demotion'' strategy for page migration, which views memory system fattened and migrates hot memory regions into top-tier memory directly. Different from \name, Memory-tiering views memory system hierarchically, which requires at most three migration to put a memory region into top-tier memory. We study the effectiveness of flatten view by implementing \name with hierarchical view.  Specifically, Memory-tiering migrates pages has cross CPU sockets accesses at the end of the first profiling interval, and promotes/demotes pages within the same memory socket at the end of the second profiling interval. For a cross socket accessed hot page, it needs three profiling interval to get top memory tier. 

%We use adaptive memory profiling in \name to guide memory regions migration and compare the efficiency of flatten view and hierarchical view. Figure~\ref{fig:migration_mode} shows the result. Overall, the flatten view performs 20\% better than hierarchical view. This is because flatten view can promote hot memory region quickly. Such that, the top-tier memory can be used batter. 

\name uses a flat view on multi-tiered memory systems, and adopts the ``fast promotion but slow demotion'' strategy. To evaluate the effectiveness of this strategy, we change \name to use a hierarchical view, where hot pages need multiple profiling intervals to reach the fastest memory. Figure~\ref{fig:migration_mode} shows that the flat view performs 20\% better than the hierarchical view because the fastest memory is used more effectively. 
%the flatten view promotes hot memory regions quickly. As a result, the fastest memory can be used more effectively.


\begin{figure}[t!]
    \centering
        \includegraphics[width=0.9\columnwidth]{figures/diff_view.pdf}
        \vspace{-5pt}
        \caption{Comparison between flatten- and hierarchical view-based migration. Performance speedup is calculated based on the performance of first-touch NUMA.} 
        \label{fig:migration_mode}
\end{figure}

\end{comment}

%\textcolor{jie2}{Performance speed up of flatten view and hierarchical view over first-touch NUMA with workloads in table~\ref{tab:app_details}.}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Effectiveness of Migration Mechanism}
\label{sec:eval_migration_mechanism}
%We further evaluate the performance of adaptive migration mechanism used in \name and \textit{move\_pages()} in Linux with three micro-benchmarks, which performs matrix read, matrix in-place update and matrix write. Figure~\ref{fig:migration} shows the result. For migration between first two tier memories (i.e., fast memory), adaptive page migration performs 40\%, 23\%, and -0.5\% better than \textit{move\_pages()}, for those pages with read-only, 50\% read, and write-only respectively. The same trend shows in migration between the first and the third memory tiers (i.e., local DRAM and local PM), and first and the forth memory tier (i.e, local DRAM and remote PM). For read-intensive pages, the adaptive migration mechanism bring performance benefit because of asynchronous page copy. For write-intensive pages, the adaptive migration mechanism performs slightly worse than \textit{move\_pages()} since the adaptive page migration has penalty of tracing the dirtiness during the migration.  

We use three microbenchmarks to evaluate the migration mechanisms in \name, Nimble~\cite{Yan:2019:NPM:3297858.3304024}, and \textit{move\_pages()} in Linux: sequential read-only, 50\% read (i.e., a sequential read followed by an update on an array element), and 100\% sequential write on a 1GB array. The array is allocated and touched in a memory tier, and then migrated to another. %To evaluate Nimble, we enable all performance optimization techniques in Nimble for the best performance. 
Figure~\ref{fig:migration} shows the results. Migrating pages between the tiers 1 and 2, \name's mechanism performs 40\%, 23\%, and -0.5\% better than \textit{move\_pages()}, and performs 26\% 4\% and -6\% better than Nimble, for the three benchmarks respectively. We see the same trend in other tiers. In general, for read-intensive pages, \name's mechanism brings large benefit; %because of asynchronous page copy; 
for write-intensive pages, \name performs similar to \textit{move\_pages()} and Nimble. %because of the overhead of tracking page dirtiness.



\begin{figure}[t!]
    \centering
        \includegraphics[width=\columnwidth]{figures/migration.pdf}
        \caption{Performance comparison between Nimble, $move\_pages()$ and \name. The performance is normalized by the performance of $move\_pages()$.}
        \label{fig:migration}
\end{figure}

%\textcolor{jie}{Performance speed up of adaptive page migration in \name and advanced page migration mechanism in~\cite{Yan:2019:NPM:3297858.3304024} over \textit{move\_pages()} in Linux with microbenchmarks.}


==> text/intro_old.tex <==
\section{Introduction}
\label{sec:intro}

%multi-tier is already there: NUMA and caches, now NVM adds extra challenges: lowest tier > 1 TB. 
Memory hierarchy has continued deepening to cope with ever-increasing demands from applications. Multi-tier memory systems that started from multi-socket non-uniform memory access (NUMA) architecture is now a de-facto solution for building scalable and cost-effective memory systems. For instance, the Amazon EC2 High Memory Instance has three DRAM-based memory tiers built upon eight NUMA nodes, providing up to 12 TB memory~\cite{amazon_high_mem_inst}. Recently, the commercial availability of new memory devices, such as high-bandwidth memory (HBM) and high-density persistent memory (PM), started expanding a new dimension of multi-tier memory systems. A multi-tier memory system implemented with heterogeneous memories and NUMA architecture can easily exceed two memory tiers. Top tiers typically feature lower memory latency or higher bandwidth but smaller capacity, while bottom tiers feature high capacity but lower bandwidth and longer latency. When high-density PM is in use, e.g., Intel's Optane DC persistent memory~\cite{Optane:blogreview}, a multi-tier large memory system could enable terabyte-scale graph analysis~\cite{vldb20_sage,optane_utexas19,peng2018graphphi}, in-memory database services~\cite{Andrei:2017:SHA:3137765.3137780,vldb21:ai_pm,ucsd_otpane:fast2020}, and scientific simulations~\cite{pm-octree:sc17,ics21:memoization} on a single machine.

%hardware cache is insufficient. 1. cache perf 2 loss on memory capacity
Muti-tier memory systems can be managed transparently by hardware, e.g., Intel's Optane can configure DRAM as a direct-mapped cache for PM. Such hardware supports require no application modifications or OS changes, and naturally, are often the first option to be explored on a new system. However, cache-like mechanisms rely on good data locality to gain performance. Indeed, applications with low data locality have shown unsatisfactory performance on such systems due to the extra overhead in managing cache~\cite{peng2019} and write amplification~\cite{nvmw21:dram-cache}. Another shortcoming of cache mechanisms is the loss of sizable memory capacity. Unlike processor caches, which are often in MBs, PM-based memory systems, e.g., Intel Cascade Lake processor, could contain hundreds of GB capacity in DRAM tiers.

%current kernel is insufficient. ref to . link to tracking TB pages, data migration.
Software-based page management can leverage multi-tier large memory systems more efficiently than hardware mechanisms because it can gain deeper insights into memory access patterns.
%\textcolor{red}{because they can gain deeper insights into applications' requirements on data. Currently, kernel solutions still rely on swapping.} 
Most of software solutions~\cite{Agarwal:2017:TAP:3037697.3037706, intel_mem_optimizer, memory_tiering, atc21_autotiering,autonuma_balance} consist of three components -- a profiling mechanism, a migration policy, and a migration mechanism. A profiling mechanism is critical for identifying performance-critical data in applications and is often realized through tracking page accesses. A migration policy chooses candidate pages to be moved to top tiers. Finally, the effectiveness of a page management solution directly depends on whether its migration mechanism can move pages across tiers at low overhead.

\textcolor{red}{(Dong: why cannot the traditional systems work?)}
\begin{itemize}
    \item \textcolor{red}{Overhead control (region-based and one sample per region) --> (\#scan based);}
    \item \textcolor{red}{The profiling process is slow to capture memory access patterns. The event-driving, not time-driving.}
    \item \textcolor{red}{Lack the support of huge page: accommodate huge page migration; merge/split a mixture of huge and regular pages; profiling huge pages.}
    \item \textcolor{red}{discuss why the global view (we must use a holistic approach)}
\end{itemize}

\textbf{Problems in profiling.} 
%The existing solutions~\cite{Agarwal:2017:TAP:3037697.3037706,kleio:hpdc19,Dulloor:2016:DTH:2901318.2901344,intel_mem_optimizer,memory_tiering,  Kannan:2017:HOD:3079856.3080245,asplos21:kloc,asplos19_softwarefarmem,autonuma_balance,pldi19:panthera,sc18:wu,Yu:ics17} have fundamental limitation to be applied on multi-tiered large memory systems because of (1) non-scalable, low-quality memory profiling mechanisms and (2) unawareness of rich memory tiers in page migration policies. 
Existing memory profiling mechanisms~\cite{Hirofuchi:2016:RHV:2987550.2987570,Kannan:2017:HOD:3079856.3080245,asplos19_softwarefarmem,asplos06_tracing_pagefault} manipulate specific bits in page table entries (PTEs) to track memory accesses at a per-page granularity. The profiling overhead scales linearly with the number of tracked pages. Our evaluation shows that tracking millions of pages could take several seconds -- too slow to respond to time-changing access patterns, and causes 20\% slowdown in TPC-C against VoltDB~\cite{voltdb}. Some solutions~\cite{Agarwal:2017:TAP:3037697.3037706, intel_mem_optimizer,memory_tiering, autonuma_balance, damon, middleware19_profiling} only profile a small set of randomly-chosen pages based on PTE manipulation or performance counters, or heavily rely on the user to configure the profiling method to reduce profiling overhead. However, such a strategy compromises profiling quality and may miss frequently-accessed pages and time-changing access patterns.

\begin{comment}
Table~\ref{tab:prof_limitation} reports the average number of hot pages detected by Thermostat~\cite{Agarwal:2017:TAP:3037697.3037706}, AutoTiering~\cite{atc21_autotiering}, and \name (our solution) in all profiling intervals of running TPC-C against VoltDB with 300GB memory footprint (see setup details in Table~\ref{tab:app_details}). With the same profiling overhead (5\%), Thermostat and AutoTiering identify 40\% and 60\% fewer hot pages than a profiling mechanism (\name) that does not use randomly selected pages, resulting in 8\% and 17\% lower performance. Finally, none of these existing solutions capture temporal data locality.
\end{comment}

%\input tables/motivation

%To make performance comparison fair, the three systems \textit{use the same page migration method}. Recent works~\cite{memory_tiering, atc21_autotiering} inherit profiling method in AutoNUMA. 

%\textcolor{jie}{We further use giga update operations per second (GUPS)~\cite{gups} as microbenchmark to evaluate the profiling efficiency. Specifically, we use 16 threads to randomly update 512 GB dataset. As figure~\ref{fig:motivation} . We set the profiling overhead as less than 5\% for different profiling methods.  Figure~\ref{fig:motivation} shows the hot pages captured by different profiling methods.}

Figure~\ref{fig:motivation} compares multiple profiling methods in Thermostat~\cite{Agarwal:2017:TAP:3037697.3037706}, AutoTiering~\cite{atc21_autotiering}, DAMON~\cite{damon, middleware19_profiling}, and our method. These profiling methods represent state-of-the-art. We use the GUPS~\cite{gups} benchmark with 512GB working set and have priori knowledge on which pages are accessed at least twice in a profiling interval (i.e., hot pages). In this workload, hot pages remain stable throughout the execution. We report profiling recall (i.e., the ratio of the number of correctly detected hot pages to the number of hot pages identified by priori knowledge) and profiling precision (i.e., the ratio of the number of correctly detected hot pages to the number of total detected hot pages including mis-identified hot pages). With the same profiling overhead (5\%), Thermostat and AutoTiering take long time to identify hot pages (see Figure~\ref{fig:motivation}). DAMON takes shorter time but about 50\% of hot pages detected by DAMON are actually not hot. Because of low profiling quality, DAMON, Thermostat, and AutoTiering perform at least 15\% worse than our method. In general, there is a lack of scalable and high-quality profiling mechanism for large memory systems. %There is a lack of an efficient methodology to maximize profiling quality without paying large profiling overhead.


%\textcolor{red}{Figure~\ref{fig:motivation} reveals the average number of hot pages detected by Thermostat~\cite{Agarwal:2017:TAP:3037697.3037706}, AutoTiering~\cite{atc21_autotiering}, and DAMON~\cite{damon, middleware19_profiling} in all profiling intervals of running the benchmark GUPS~\cite{gups} with 512GB working set.  With the same profiling overhead (5\%), Thermostat and AutoTiering identify 40\% and 60\% fewer hot pages than a profiling mechanism (\name) that does not use randomly selected pages, resulting in 8\% and 17\% lower performance. Finally, none of these existing solutions capture temporal data locality.}


\begin{figure}[t!]
    \centering
        \includegraphics[width=\columnwidth]{figures/access_pattern.pdf}
        \vspace{-15pt}
        \caption{\textcolor{red}{figure format is not acceptable. }Comparison of different memory profiling methods in terms of their effectiveness of identifying frequently accessed pages (hot pages). The profiling overhead is set as 5\% of total execution time.}
        \label{fig:motivation}
        %\vspace{-5pt}
\end{figure}

\begin{comment}
\begin{figure}
    \begin{subfigure}
        \includegraphics[width=0.9\columnwidth]{figures/motivation1.pdf}
        %\subcaption[1]{The recall of different memory profiling methods for finding hot pages. }
    \end{subfigure}
    \begin{subfigure}
        \includegraphics[width=0.9\columnwidth]{figures/motivation2.pdf}
        %\subcaption[2]{The precision of different memory profiling methods for finding hot pages. }
    \end{subfigure}
    \caption{\textcolor{dong}{Comparison of different memory profiling methods in terms of their effectiveness of identifying hot pages}.}
    \label{fig:motivation}
    %and so on
\end{figure}
\end{comment}
\textbf{Problems in migration.} Existing solutions to multi-tiered memory are built upon an abstraction extended from traditional memory hierarchy, where page migration occurs between two neighboring tiers. However, such abstraction could limit multi-tiered memory systems. First, migrating pages from the lowest to the top tier, at tier-by-tier steps, takes time, e.g., tens of microseconds for a 4K page. Also, frequent data movement across tiers is needed to accommodate time-changing access patterns, different from occasional swapping between memory and storage.

%4 principles for effective multi-tier systems:
To leverage a multi-tier large memory system efficiently, we argue that the following four principles must be upheld.

\begin{itemize}[leftmargin=*,noitemsep,topsep=0pt]
\item \textit{Scalable quality-aware profiling.} Formal metrics that quantify performance impact from pages need to be established to guide page selection for profiling. By only tracking the most performance-critical pages at a time, a solution can guarantee adaptiveness to time-changing patterns and controlled overhead.

\item \textit{Global view of memory regions in all tiers.} Only tracking data in the fastest tier is insufficient because large memory regions are forced to reside in lower tiers even though they may contain small but performance-critical subregions. This is particularly true on terabyte-scale systems where data in the top tiers can only accommodate a small portion of total working sets and thus insufficient to provide a comprehensive view of system-wide data. Thus, a global view of all memory regions in all tiers is crucial.

\item \textit{Tier-bypassing migration.} Emerging large-memory systems feature multiple tiers. Migration through neighboring tiers is too slow. Instead, performance-critical pages should be promoted to the top tier bypassing intermediate tiers, i.e., pages in all slower tiers have equal chances to be promoted to the fastest tier. Victim pages evicted from the top tier should be progressively demoted into the next available lower tier instead of the bottom tier as in the  existing swapping-based solution in Linux~\cite{autonuma_balance} (i.e., AutoNUMA) because these pages are still likely to be accessed.

\item \textit{Pattern-aware migration mechanism.} The page migration mechanism includes multiple stages. Parallelism between stages is often ignored. Considering read/write patterns of page accesses, such parallelism can be exposed, which is critical to improve page migration performance on multi-tiered memory with frequent page migration.
%\textcolor{red}{leverage pattern information to enable higher parallelism for higher performance, e.g., read-intense lower consistency overhead...... Due to the diversity in memory tiers, a single migration mechanism is no longer sufficient. Instead, depending on the access patterns to migrated pages and the characteristics of the destination memory tier, proper migration schemes should be derived accordingly to limit the impact on application performance.}
 
\end{itemize}

%our contributions
In this work, we contribute a software-based page management solution called \name that realizes the four principles on terabyte-scale multi-tier memory. 

\name maintains a flat global view of all memory regions in all memory tiers. Profiling quality and overhead are distributed proportionally according to a memory region's importance. Memory regions with a higher impact on performance are tracked with higher fidelity, i.e., more pages are selected for profiling. In particular, \name uses spatial and temporal variation as the key metrics to quantify the performance impact of a memory region. Over time, \name adaptively merges and splits memory regions based on their similarity in spatial and temporal locality so that pages in a memory region have similar access patterns.

\name uses the ``fast promotion slow demotion'' policy for page migration. Hot pages identified in all lower tiers can be directly promoted to the top tier, minimizing data movement through tiers. When a page is migrated out of the top tier to accommodate more important pages, the page will be moved to the next lower tier with available space. \name dynamically chooses from an asynchronous page copy-based scheme and a synchronous page migration scheme, based on the read/write pattern of the migrated page, to minimize migration time. 


%our results
\textbf{Evaluation.} We rigorously evaluated \name against seven state-of-the-art solutions, including two industry-quality software solutions (Intel Memory-optimizer~\cite{intel_mem_optimizer} and Intel Memory-tiering~\cite{memory_tiering}), two state-of-the-art solutions (AutoTiering~\cite{atc21_autotiering} and HeMem~\cite{sosp21_hemem}), an existing solution in Linux (AutoNUMA~\cite{autonuma}), a hardware-based solution (Optane Memory Mode), and first-touch NUMA. \name is also compared against two kernel-based page migration solutions (the ones in Linux and Nimble~\cite{Yan:2019:NPM:3297858.3304024}). \name outperforms Intel memory-optimizer, Intel memory-tiering, AutoTiering, AutoNUMA, Memory Mode, first-touch NUMA and HeMem by 32\%, 22\%, 20\%, 25\%, 24\%, 20\%, and 24\% on average. \name outperforms the Linux and Nimble migration approaches by 40\% and 36\% for read-intensive workloads, and has similar performance for write-intensive workloads.



==> text/intro_old_old.tex <==
\section{Introduction}
\label{sec:intro}
%\textcolor{red}{paragraph 1: explain the background of big memory systems. Give two example systems and big memory applications, including big graph, big database, and HPC applications.}

%\textcolor{red}{(The following paragraph can be simplified.)}
Large memory systems with multiple TBs or more are emerging. These systems are driven by the emergence of memory-consuming applications and recent advances in memory technologies. From the application perspective, we see terabyte-scale graph analysis~\cite{vldb20_sage,optane_utexas19,peng2018graphphi}, large in-memory database services~\cite{Andrei:2017:SHA:3137765.3137780,vldb21:ai_pm,ucsd_otpane:fast2020}, and extreme-scale scientific simulations~\cite{pm-octree:sc17,peng2018siena,ics21:memoization}. From the memory technology perspective, we see recent Intel's Optane DC persistent memory (PM) supports up to 12TB on a two-socket  machine~\cite{Optane:blogreview}. The trend of large memory systems will continue, as the applications work on increasingly large working sets, and technological advances decrease memory cost and increase memory density.
%\textcolor{red}{(Dong TODO: The use case and problem solved are a bit unclear: many assumptions about hardware and workloads have to hold before Titan becomes necessary)}


The existing large memory systems are often characterized with more than two memory tiers, and different tiers show different memory latencies and bandwidths. Such rich memory heterogeneity, built upon various memory technologies and multi-socket non-uniform memory access (NUMA) architectures, provides a scalable and cost-effective solution to enable large memory systems. %For example, on an Intel's Optane-based two-socket machine, DRAM and Optane create two tiers; the NUMA effect on this machine adds the third tier to scale up memory. 
For example, the Intel Optane-based machine has four memory tiers where Optane and DRAM create two tiers and the NUMA effect creates another two, providing up to 12 TB memory. 
%\textcolor{jie2}{(from jie: should we delete the following sentence? this sentence does not discuss multiple memory tier.) 
Also, since DRAM is more costly but provides higher bandwidth and lower latency than Optane, DRAM is used as a small cache to Optane for lower production cost and higher performance. 
%For example, on an Intel's Optane-based two-socket machine, DRAM (as fast memory) works with Optane persistent memory as a software- or hardware-managed cache to address relatively low performance of the persistent memory (as slow memory), creating two memory tiers, and the NUMA effect on this machine adds the third tier.
Take another example. The Amazon EC2 High Memory Instance has three DRAM-based memory tiers built upon eight sockets and NUMA, providing up to 12 TB memory~\cite{amazon_high_mem_inst}. Richness in NUMA nodes in this machine is needed to scale up memory. In contrast, the traditional memory systems with smaller memory capacity are often equipped with at most two memory tiers.


%\textcolor{red}{paragraph 2: common problem of the current system designs. We add a table to show the large profiling overhead of the current methods or poor migration performance of the current methods. Our baselines: Intel mem-tiering Linux kernel module, Michigan paper (?), and xxxx.}


%To optimize a heterogeneous memory system for performance, one would ideally place the hottest data in the fastest memory node (in terms of latency or bandwidth) until that node is full, the next hottest data would be filled into the second-fastest node up to its capacity, and so on. As a program executes, its data would be periodically assessed for hotness and re-organized to maximize performance. For emerging software-controlled heterogeneous memory systems, hotness detection and migration requires effective software mechanisms and policies to determine data reuse and control data migration.


Making effective, transparent use of the multi-tiered large memory system requires a page management system. 
%based on which the large-memory application can make the best use of the fastest memory (in terms of latency or bandwidth) for high performance and slow memories for large memory capacity. 
%As a program executes, the page management system would periodically assess program data for hotness and re-organize them to maximize performance.
Because of limited capacity in fast memories, the application with large memory footprint has to spread its pages across memory tiers. The application can have varying memory access patterns, which demands a page management system to assess pages for hotness and distribute them between memory tiers to maximize performance. There are software-based page management solutions~\cite{Agarwal:2017:TAP:3037697.3037706, intel_mem_optimizer, memory_tiering, atc21_autotiering,autonuma_balance} where the tiered memories share the physical address space and a system software is in charge of page management. The software-based page management consists of at least three components: a memory profiling mechanism, a page migration policy, and a page migration mechanism. The memory profiling mechanism is needed to track page accesses and assess pages for hotness; The page migration policy and mechanism shuffle pages between tiers to maximize fast-memory accesses. 
%\textcolor{red}{Such optimal memory management should be able to place each data object in the proper memory device in proper time so that the performance penalty from the slow auxiliary memory device is concealed.} \textcolor{red}{a migration mechanism seeks to shuffle pages between tiers to maximize fast-memory accesses.}
%Such a page management system for multi-tiered systems is not implemented in commercial hardware, given the potential cost of extensive modification of cache hierarchy and memory controller~\cite{}. \textcolor{red}{(how about the memory node in Optane)} 





\textbf{Problems.} 
The existing solutions~\cite{Agarwal:2017:TAP:3037697.3037706,kleio:hpdc19,Dulloor:2016:DTH:2901318.2901344,intel_mem_optimizer,memory_tiering,  Kannan:2017:HOD:3079856.3080245,asplos21:kloc,asplos19_softwarefarmem,autonuma_balance,pldi19:panthera,sc18:wu,Yu:ics17} have fundamental limitation to be applied on multi-tiered large memory systems because of (1) non-scalable, low-quality memory profiling mechanisms and (2) unawareness of rich memory tiers in page migration policies. 
%are not scalable on a large memory system because of expensive page profiling and migration mechanisms; Those solutions are also designed for a system with no more than two memory tiers and do not consider more than one memory as a target for page migration. 


The existing memory profiling mechanisms for heterogeneous memory~\cite{Hirofuchi:2016:RHV:2987550.2987570,Kannan:2017:HOD:3079856.3080245,asplos19_softwarefarmem,asplos06_tracing_pagefault} are commonly based on the manipulation of specific bits in page table entries (PTE) to track memory accesses. This mechanism accurately
captures memory accesses at a per-page granularity, matching established abstraction in operating systems (OS) for data migration and memory management.
%\textcolor{red}{(Dong TODO: A better motivation (beyond "other people have published on this") and discussion of why paging and the virtual memory subsystem are the right way to solve this problem would also make the paper much stronger)}
%This mechanism involves flushing TLB and triggering page faults, which is expensive. 
\textcolor{check}{%However, using this mechanism to track memory accesses  the scale of millions of pages (even using 2MB huge page size) accurately requires large runtime overhead. 
However, the profiling overhead grows arbitrarily as the number of pages to be tracked increases. For example, the overhead of tracking memory accesses at the scale of millions of pages takes multiple seconds, which is too slow to respond to time-changing access patterns. Such a large overhead causes over 20\% performance slowdown in TPC-C against VoltDB~\cite{voltdb} (see Table~\ref{tab:app_details}) in our evaluation.} %\textcolor{red}{when the time for tracking target pages exceeds the user-defined time interval.}
%\textcolor{dong}{multiple seconds} \textcolor{red}{(Jie TODO: replace the above number with a concrete application to quantify profiling overhead)}, which is not scalable and \textcolor{dong}{too slow to respond to time-changing access patterns.}
%\textcolor{red}{Dong TODO: Tens of seconds of what? Latency, presumably, but what sort of latency? Pauses for the whole system, or traversal time until a promotion/demotion decision is made? Who perceives this latency?} 
To avoid the large overhead, some solutions~\cite{Agarwal:2017:TAP:3037697.3037706, intel_mem_optimizer,memory_tiering, autonuma_balance} selectively profile memory pages in randomly-chosen small memory regions. These solutions trade profiling quality for low overhead, but lose track of frequently accessed pages and time-changing access patterns.
%(From jie: Does "time-changing access patterns" has the similar meaning as "temporal data locality"? I suggest the above sentence can be changed as "but lose the track of frequently accessed pages in a comprehensive view on large memory systems." )
These solutions also fail to capture similarity of access patterns across regions to merge regions and reduce overhead; Furthermore, all profiling mechanisms do not capture temporal data locality very well, because they do not correlate time-consecutive profiling results. 
%%These solutions also partition the address space into fixed-size memory regions. These solutions profile one sample page out of each memory region to represent memory access patterns of the whole region. 
%Fixing the size of memory regions, these solutions suffer from the potential problem of using a singe page to mis-represent memory access patterns of the whole region; 
%%Fixing the size of memory regions and using a single page per region for profiling introduces the question of whether the page samples are representative of the memory regions. 

\input tables/motivation

To illustrate the above random profiling problem, Table~\ref{tab:prof_limitation} quantifies the effectiveness of profiling mechanisms in Thermostat~\cite{Agarwal:2017:TAP:3037697.3037706}, AutoTiering~\cite{atc21_autotiering}, and \name (our solution) using TPC-C against VoltDB with 300GB memory footprint (see Table~\ref{tab:app_details}). To make performance comparison fair, the three systems \textit{use the same page migration method}. 
%Recent works~\cite{memory_tiering, atc21_autotiering} inherit profiling method in AutoNUMA. 
\textcolor{check}{Table~\ref{tab:prof_limitation} 
reports the average number of identified hot pages (i.e., the most frequently accessed pages) among all profiling intervals.}
%%%reports the number of identified hot pages (i.e., the most frequently accessed pages) among all profiling intervals. %identified to move to the fastest memory tier. 
With the same profiling overhead (5\%), Thermostat and AutoTiering identify 40\% and 60\% less hot pages than a highly optimized profiling mechanism in \name. Just because of low profiling quality, Thermostat and AutoTiering perform 8\% and 17\% worse respectively. 

In general, there is a lack of scalable and high-quality profiling mechanism for large memory systems. There is a lack of an efficient methodology to maximize profiling quality without paying large profiling overhead.
%explore the tradeoff between profiling overhead and quality.

%There is a pressing need to study the scalability of system software on large memory systems 
%different from the middleware paper: (1) no histogram; (2) no consideration of mem accesses (only access or not); (3) dynamical change of the number of sample regions. In general, sampling quality is not good enough;

From the perspective of page migration strategy, the existing solutions are built upon a memory abstraction of two-tiered memory: The page migration happens from one tier to the other. An extension to the above policies for multiple tiers is to build a hierarchical view of the multiple memory tiers according to their performance difference, as in the traditional memory hierarchy. Based on this hierarchical view, the page migration happens between two neighboring tiers in the hierarchy. Although this policy works well in the traditional memory hierarchy, it cannot work well in the multi-tiered memory systems, because of two reasons. %\textcolor{jie2}{(From jie: We need to discuss the following points.) (1) Traditional caching algorithms are useful only when the performance difference between devices is at least 10x, while the gap between memory tiers in large memory system is not that big. Tier-by-tier page migration in large memory system can not bring performance benefit. For example, as shown in figure~\ref{fig:multi-tiered-mem}, the performance gap between two memory tiers in Optane-based memory system is less than 2x.
(1) Data movement from the slowest memory tier to the fastest takes long time (at the granularity of tens of microseconds for a 4K page). 
%This data movement time in multi-tiered memory systems is much longer than that in the processor's cache hierarchy. 
Such a long time of data movement is difficult to be hidden and hence causes large performance loss. (2) Data movement across the memory tiers happens frequently to accommodate time-changing memory-access patterns, much more frequently than that between memory and storage. Hence reducing data movement time across the memory tiers is more pressing than that between memory and storage.

%point 1: profiling overhead (Umich paper) is too large on big mem when profiling all mem pages; Profiling is not accurate (Intel tiering); %point 2: the migration method is not aware of multi-tiered auto-numa balance

%However, making effective, transparent use of slow memory to reduce cost without substantial performance loss is challenging. Any memory placement policy must estimate the performance degradation associated with placing a given memory page in slow memory, which in turn requires some method to gauge the page access rate. Lack of accurate page access rate tracking in contemporary x86 hardware makes this task challenging. Moreover, as we will show, naive policies to place pages into slow memory based on existing hardware-maintained Accessed bits are insufficient and can lead to severe performance degradations.



%\textcolor{red}{Paragraph 3: our principle (using a ``quantified'' approach) (?adaptiveness to quantify and minimize the profiling overhead or migration overhead). distinguish between migration interval and profiling window size.}
\textbf{Goal and Insights.}
The goal of this project is to design a page management system that automatically migrates pages between memory tiers to maximize fast-memory accesses with low overhead. Our major drive is a shift from non-scalable, empirical, and narrow-scoped designs for the traditional simple-tiered memory system to a scalable, quantified, and general design for the multi-tiered large memory system. 
%The goal of this project is to design a memory-disaggregation-friendly managed runtime that can provide superior efficiency to all managed cloud applications running in a memory-disaggregated datacenter. Our major drive is an observation that shifting our focus from low-level, semantics-agnostic optimizations (as done in prior work) to the redesign of the runtime that improves data placement, layout, and usage, can unlock massive opportunities.

To achieve the above goal, we have two insights. First, the memory profiling mechanism must be \textit{adaptive}, which means adaptively forming memory regions and choosing pages for profiling based on spatial and temporal variation of memory access patterns. Such adaptiveness is the key to establish a comprehensive view of memory access patterns of all memory pages \textcolor{check}{(instead of some random pages)} without large overhead; the adaptiveness should also be based on \textit{fine quantification} of profiling overhead, such that the dynamic nature of this new profiling principle does not cause large performance loss. 
%Overhead control; how to spread the alloweable number of pages across regions. quantifiable approach to strike a balance between profiling quality and overhead 


Second, the page migration in the multi-tiered memory must employ a \textit{holistic} design principle. This means that page movement is not only between neighboring tiers but also between the fastest memory and any other memory tiers, and any slow memory tier has equal opportunities to directly use the fastest memory. In other words, we use a flatten view, instead of the hierarchical view, to holistically decide which pages should be in the fastest memory for high performance. Being holistic is the key to enable effective page migration and make the best use of fast memories for high performance.


\textbf{\name.} Following the above insights, we develop \name, an application-transparent page management system that supports efficient use of multi-tiered large memory with high performance.

\name is based on four key ideas to address the memory profiling challenge: %of scalability, overhead and quality: 
adaptive memory regions, adaptive page sampling, correlation of time-consecutive profiling results, and fine-grained profiling overhead control. In particular, \textit{adaptive memory regions} can be merged or split based on the similarity of memory access patterns between regions;
\textit{Adaptive page sampling} dynamically changes the number of page samples for profiling based on the variation of memory access patterns within individual memory regions. The above two techniques aim to maximize profiling quality without increasing profiling overhead. The two techniques also capture spatial locality. \textit{Correlation of time-consecutive profiling results} aims to capture temporal locality by building a histogram of profiling results. \textit{Fine-grained profiling overhead control} is integrated with the above adaptive techniques, and dynamically enforces limits on profiling overhead. 
%to ensure the performance gains in whole system.
%\textcolor{dong}{dynamically enforces limits on performance degradation (e.g., limiting application slowdown to 5\%).}
%\textcolor{dong}{uses a quantitative approach to control profiling overhead within a constraint}. 


\name uses a strategy of ``fast promotion but slow demotion'' for page migration, following the holistic design principle. In particular,  slow memory tiers promote their hot pages to the fastest memory and compete for it based on the profiling results. This fast-promotion approach allows frequently accessed pages to be in the fastest memory for high performance without time-consuming movement along other tiers. Furthermore, when a page is migrated out of the fastest memory to accommodate more frequently accessed pages, we use a hierarchical view and migrate the page slowly to %the second-level tier in the memory hierarchy. 
lower tiers in the memory hierarchy with available space. This slow-demotion approach mitigates performance loss caused by migrating frequently accessed pages to a low memory tier. %when the fastest memory does not have space.

In addition, \name is featured with a new  migration mechanism. It dynamically decides whether copying pages should happen asynchronously or synchronously based on the memory access pattern to minimize migration overhead. 

%Recognizing performance difference between common page migration mechanisms when migrating read-intensive and write-intensive pages, \name adaptively chooses which mechanism should be used, following the adaptive design principle. 

%\textcolor{jie}{We evaluate \name using common big-data applications with large working sets (hundreds of GB to TB). Our results demonstrate that \name improves the performance of hardware managed cache, default Linux NUMA page placement solution first-touch NUMA, and Linux dynamic NUMA balancing solution AutoNUMA~\cite{autonuma_balance} by an average of 24\%, 20\%, 25\%, respectively. Furthermore, \name consistently outperforms two industry-quality page management systems (memory-optimizer~\cite{intel_mem_optimizer}, memory-tiering~\cite{memory_tiering}) and state-of-the-art multi-tierd memory management solution (AutoTiering~\cite{atc21_autotiering}) by an average of 32\%, 22\% and 20\% , respectively. }



\textbf{Results.} 
\textcolor{check}{We compare \name with six solutions, including two industry-quality software solutions (Intel Memory-optimizer~\cite{intel_mem_optimizer} and Intel Memory-tiering~\cite{memory_tiering}), a state-of-the-art solution (AutoTiering~\cite{atc21_autotiering}), an existing solution in Linux (AutoNUMA~\cite{autonuma}), a hardware-based solution (Optane Memory Mode), and first-touch NUMA. We also compare with two solutions (the existing page migration mechanism in Linux and Nimble~\cite{Yan:2019:NPM:3297858.3304024}) in terms of page migration mechanism.}
%We also compare with two solutions (Thermostat~\cite{thermostat_asplos17} and Nimble~\cite{Yan:2019:NPM:3297858.3304024}) in terms of memory profiling and page migration mechanism respectively.

\name outperforms Intel memory-optimizer, Intel memory-tiering, AutoTiering, AutoNUMA, Memory Mode and first-touch NUMA by 32\%, 22\%, 20\%, 25\%, 24\%, and 20\% on average. \name outperforms the existing page migration mechanism in Linux and Nimble by 40\% and 36\% (in terms of execution time) for read-intensive workloads, and reaches the similar performance for write-intensive workloads.
%Using the same page migration strategy and mechanism, \name outperforms Thermostat by 7\% due to superior memory profiling.




%We have evaluated Semeru using two widelydeployed systems – Spark and Flink – each with a representative set of programs. Our results demonstrate that Semeru improves the end-to-end performance of these systems by an average of 2.1× and 3.7× when the cache size is 50\% and 25\% of the heap size, application performance by an average of 1.9× and 3.3×, and GC performance by 4.2× and 5.6×, respectively, compared to running these systems directly on NVM-oF where remote accesses incur significant latency overheads. These promising results suggest that Semeru reduces the gap between memory disaggregation and managed cloud applications, taking a significant step toward efficiently running such applications on disaggregated datacenters.




%\textcolor{red}{Paragraph 4: summarize key ideas.}

%\textcolor{dong}{(robust to sampling frequency?)}




==> text/motivation_old.tex <==
\section{Motivation}
\label{sec:motivation}
High accuracy, low overhead profiling mechanism is key for managing multi-tiered large memory. We study the profiling methods in state-of-the-art works (Thermostat~\cite{Agarwal:2017:TAP:3037697.3037706}, AutoTiering~\cite{atc21_autotiering}, Linux's DAMON~\cite{damon, middleware19_profiling}) and summarize their overhead and accuracy tradeoff as follows. AutoTiering randomly choose \textcolor{red}{xxxx MB} pages for profiling to detect hot pages. Both Thermostats and DAMON maintain a list of memory regions and randomly choose one page per region for profiling. Thermostats keeps all memory regions in a fixed size while DAMON dynamically splits and merges memory regions to improve profiling quality -- they control profiling overhead by changing the number of memory regions.

We compare the profiling methods in these works with \name by running the GUPS~\cite{gups} benchmark with a 512GB working set on the four-tier memory system in Figure~\ref{fig:multi-tiered-mem}. We know a priori page hotness in each profiling interval during execution. Figure~\ref{fig:motivation} reports profiling $recall$ (i.e., the ratio of the number of correctly detected hot pages to the number of hot pages identified by priori knowledge) and profiling $precision$ (i.e., the ratio of the number of correctly detected hot pages to the number of total detected hot pages including mis-identified hot pages). 
%We have priori knowledge on which pages are accessed at least twice in a 5-sec. profiling interval (i.e., hot pages).  In this workload, hot pages remain stable throughout the execution. 

With the same profiling overhead (5\%), Thermostat and AutoTiering take long time to reach high recall (i.e., slower to identify hot pages) in Figure~\ref{fig:motivation}.a, because their randomness in page sampling and the formation of memory regions cause uncontrolled profiling quality. DAMON takes shorter time in Figure~\ref{fig:motivation}.a, but about 50\% of hot pages detected by DAMON are actually not hot (see~\ref{fig:motivation}.b), because of its ad-hoc design of forming memory regions and slow response to the variance of memory access patterns. Due to low profiling quality. DAMON, Thermostat, and AutoTiering perform 15\% worse than \name.

%In general, there is a lack of high-quality and scalable profiling mechanism for large memory systems. %There is a lack of an efficient methodology to maximize profiling quality without paying large profiling overhead.

\begin{figure}[t!]
    \centering
        \includegraphics[width=\columnwidth]{figures/access_pattern.pdf}
        \vspace{-15pt}
        \caption{Comparison of different memory profiling methods in terms of their effectiveness of identifying hot pages.}
        \label{fig:motivation}
        %\vspace{-5pt}
\end{figure}

%The profiling overhead is set as 5\% of total execution time.

==> text/overview_old.tex <==
\section{Overview}
\label{sec:overview}
%\textcolor{red}{(Add an overview section). Define profiling window, migration window, and sleep time. Define the profiling overhead budget.}

%We implement \name in the Linux xxxxx kernel.  \textcolor{red}{(add a few sentences on how a user would use \name. Use the following paragraph from the Thermostat paper as an example.)} ``Thermostat can be controlled at runtime via the Linux memory control group (cgroup) mechanism [38]. All processes in the same cgroup share Thermostat parameters, such as the sampling period and maximum tolerable slowdown.''

%All application processes whose page management is conducted by \name share parameters, such as the profiling interval, migration interval, and profiling overhead target.
%\textcolor{red}{Jie TODO: check the correctness and completeness of the overview section.}

%\textcolor{dong}{\name aims to support multi-tiered large memory systems, addressing the limitations in existing memory profiling and migration mechanisms in Linux (the state-of-the-art solutions).} 

\textcolor{dong}{We rethink of memory profiling and migration to support multi-tiered large memory systems.} 

\textcolor{dong}{\textbf{Existing profiling mechanism in Linux} (i.e., DAMON) is the most effective up to now. It splits the virtual memory space of a given process into memory regions, and periodically profiles memory accesses and migrates pages. In each profiling interval, DAMON randomly profiles one 4KB page (instead of all pages) per memory region to capture spatial locality.} 
%This region-based profiling strategy mainly captures spatial locality in each region.}

\textcolor{dong}{To control the profiling overhead, DAMON asks the user to specify the maximum number of memory regions for profiling, and then dynamically merges and splits memory regions.  DAMON merges two neighbor memory regions if their profiling results in a time interval differ less than 10\%. DAMON splits each memory region into two random regions to improve profiling quality, when the number of memory regions is less than a half of the maximum number of memory regions.} 

%One main property of our technique that differentiates it from other page table access bit based schemes is its support of the bounded trace overhead. For this property, we split the virtual memory space of a given process into sub-regions and monitor only sampled pages in each memory region instead of every page. Users can, thus, control the upper-bound of tracing overhead by limiting the maximum number of regions. Furthermore, it minimizes the errors caused by the sampling and dynamic change of the data access pattern by adaptively restructuring the regions so that each region covers only memory regions with unique data access patterns that are different from adjacent regions. In this way, our technique keeps the worst-case tracing overhead under a user-defined bound regardless of the size of target workloads, while preserving its output quality as high as possible.

\textcolor{dong}{\textbf{Limitations in existing mechanism.} DAMON has five limitations, making it less efficient to support the multi-tiered large memory systems.} 

\begin{enumerate}[leftmargin=*,noitemsep,topsep=0pt]
    \item \textcolor{dong}{The control of profiling overhead is not directly connected with the profiling mechanism (i.e., scanning PTEs), but connected with the number of memory regions with a constraint that the number of profiling pages (or the number of PTE scans) in each memory region must be one. This constraint compromises profiling quality.}
    
    \item \textcolor{dong}{Splitting memory regions is ad-hoc. The random split can lead to useless profiling when the new memory regions after splitting have the similar memory access patterns.}

    \item \textcolor{dong}{The process of forming memory regions can be slow to capture access patterns, because of the time constraint in the profiling interval. This is problematic in a large  memory system with many memory regions to split and merge.}
    
    \item \textcolor{dong}{DAMON does not consider temporal locality well.} 
    
    \item \textcolor{dong}{Lack of support for profiling huge pages.} 
    %\textcolor{dong}{In the case of using huge pages, a memory region can be a mixture of 4KB pages and huge pages. Profiling at 4KB pages lacks the support of huge pages.}
\end{enumerate}
   
\textcolor{dong}{Like DAMON in Linux, \name partitions the virtual address space of a process into memory regions for profiling, and dynamically merge and split them.}

%\textcolor{dong}{Different from in DAMON, the profiling overhead control in \name is decoupled from the number of memory regions. This enables new memory merging/splitting schemes, addressing the limitations of 1 and 2.}

\textcolor{dong}{Different from DAMON, the profiling overhead control in \name is designed by considering the total number of PTE scans in all memory regions (Section~\ref{sec:overhead_control}). As a result, \name has freedom to perform PTE scan multiple times for a page or multiple pages in a memory region in a profiling interval (Section~\ref{sec:page_sampling}). 
%as long as the total number of PTE scans does not violate a constraint to meet the user-specified overhead requirement. Having such flexibility in profiling enables higher profiling quality.
Having such flexibility provide opportunities to re-distribute sampling quotas between memory regions under a fixed profiling overhead to improve profiling quality, addressing the limitations of 1 and 2.} %We discuss the above points in Section~\ref{sec:profiling}.} 

\textcolor{dong}{\name uses performance counter-assisted PTE scanning to address the limitation 3 (Section~\ref{sec:hybrid_profiling}).}

%By default, a memory region is a contiguous address space mapped by a last-level page directory entry (PDE). This indicates that in a typical five-level page table, the memory region size is 2MB by default. During program execution, whenever a last-level PDE is set as valid by OS, the corresponding memory region is subject to profiling. \textcolor{dong}{Like DAMON, memory regions in \name can be dynamically merged and split. Different from DAMON, \name addresses the above five limitations for the large memory systems, discussed as follows.}

%\textcolor{dong}{\name uses performance counter-assisted PTE scanning to address the limitation 3 (see Section~\ref{sec:hybrid_profiling}). In the largest memory tier, \name uses performance counters to identify memory region candidates to be profiled using PTE scanning. The performance counter technique use a performance event-driven approach (not time-driven as in DAMON) for performance profiling. This enables faster identification of hot memory regions.}

%\textcolor{jie2}{The goal of \name is to provide an application-agnostic memory management for big memory. \name contains three major components, including adaptive memory profiling (\S\ref{sec:profiling}), holistic page migration(\S\ref{sec:migration}), and memory region based migration mechanism (\S~\ref{sec:mechanism}). Figure~\ref{} shows the workflow of \name. }

%\name partitions the virtual address space into memory regions. It periodically profiles memory accesses and migrates pages. In each profiling interval, \name samples one or more pages per memory region. This region-based profiling strategy captures spatial locality in each region. Memory regions can be dynamically merged or split under the guidance of quantitative analysis on the profiling overhead. Such adjustments provide opportunities to re-distribute sampling quotas between memory regions under a fixed profiling overhead to improve profiling quality.

%When making decisions on page migration between memory tiers, \name uses a holistic approach.
\name decide page migration between memory tiers based on a ``global view'' of all memory regions (Section~\ref{sec:migration}). %\name calculates the exponential moving average of page hotness collected from all profiling intervals, based on which \name builds a histogram to get the distribution of hot memory regions in all memory tiers.
By calculating the exponential moving average of page hotness collected from all profiling intervals (\textcolor{dong}{addressing the limitation 4}), \name learns the distribution of hot memory regions in \textit{all} memory tiers. 

%%%promotes hot pages from \textit{any memory tier} to the fastest tier without going through any intermediate layers. It demotes pages \textit{tier by tier} when there is not enough space in the fast memory tiers. 


%\textcolor{red}{\name builds a histogram of memory accesses for memory regions} to capture temporal locality. The histogram includes information for all tiers and allows \name to move hot pages from any tier to the fastest memory without going through slow data movement.

%\textcolor{red}{Dong TODO: The paper jumps straight into the weeds of discussing the promotion/demotion details and mechanisms, but never says clearly that promotion and demotion happens at the granularity of regions. It would be great to make this clear early on.}


Beyond profiling, \name has innovation in migration. Guided by the new profiling techniques, \name introduces the ``fast promotion and slow demotion'' policy (Section~\ref{sec:where_to_migrate}). Also, when migrating pages, \name uses an asynchronous page-copy mechanism that overlaps page copying with application execution. This mechanism reduces the overhead of page copy, but come with the time cost of \textit{extra} page copy, because when a page is updated during copying, the page has to be copied again. The traditional, synchronous page-copy mechanism does not need extra page copy, but completely exposes the overhead of page copy into the critical path. Hence, \name uses a hybrid approach that takes advantage of both mechanisms, and selects one based on whether page modification happens during migration (Section~\ref{sec:mechanism}).  

\textcolor{dong}{To support huge pages,  \name enables page profiling at the huge page level instead of 4K-page level using the page table information; memory merging and splitting are carefully managed to be aligned with the huge page size, such that the huge page semantics is not broken (Section~\ref{sec:profile_huge_page}). The support migration of huge pages, \name lifts the constraint in Linux that huge pages cannot move across distant memory tiers and support huge-page migration based on the existing support of 4KB-page migration (Section~\ref{sec:migration_huge_page}).} 

%{To support migration of huge pages, \name lifts the constraint in Linux that huge pages cannot move across distant memory tiers because of unawareness of multiple memory tiers; \name also extends the migration mechanism to support migration of huge pages based on the existing support of 4K-page migration (Section~\ref{sec:migration_huge_page}).}

%{\name extends PTE to expose huge page identification, such that the profiling can intentionally happen at the huge page level; The merging and splitting of memory regions are also able to be aligned with huge pages (see Section~\ref{sec:profile_huge_page}). Furthermore, \name introduces the awareness of memory tiers to the memory space reserved for huge page to accommodate huge page migration across tiers (see Section~\ref{sec:migration_huge_page}). Demote to slow memory for huge pages.}

In summary, \name has three components: (1) an adaptive memory profiling mechanism with high profiling quality and constrained overhead; (2) a page-migration strategy that leverages a global view to make informed decisions; and (3) a page-migration mechanism that adapts data copy schemes based on page access patterns. 


%We depict the three components in detail as follows.
%This overhead control uses a quantified approach to bound the total number of page samples (and page scans), such that the profiling overhead is within the profiling overhead budget. Merging and splitting regions 

%Two memory regions, when their profiling results are similar, can be merged to a large memory region with fewer page samples; A memory region, when its profiling result shows large variance across page samples, can be split into two regions to improve profiling quality. Dynamically merging and splitting regions is under the profiling overhead control. This overhead control uses a quantified approach to bound the total number of page samples (and page scans), such that the profiling overhead is within the profiling overhead budget. Merging and splitting regions 

%promotes hot memory regions across memory tiers to the fastest memory based on a memory access histogram, and ,


%introduce (1) memory region, (2) profiling interval (3)migration interval
%\textcolor{jie2}{\name manages big memory system at the granularity of memory region, which is a contiguous virtual memory space. \name splits the execution of application as equal length migration interval. In each migration interval, }

%\textcolor{jie2}{In this work, we introduce an efficient profiling method which carefully select sampled pages by considering spacial and temporal locality. The profiling in \name is based on PTE access bit scanning.  The profiling method of \name has four components, including (1) adaptive memory regions selection, (2) adaptive page sampling, (3) time-consecutive profiling, and (4) fine-grained profiling overhead control. The adaptive profiler track memory access hotness with user-specified profiling overhead. Profiling happens in the granularity of memory region, which is a contiguous virtual memory space. In each memory region, the profiler samples at least one page as representative page. After consecutive scanning representative pages, the profiler reports the number of memory access for each memory region in each profiling window. With processing and analyzing history memory access information for each memory region, the profiler adaptively changes the memory region size and the number of representative pages in each memory region for next profiling window. At the end of each profiling window, the profiler stops scanning PTE to ensure profiling overhead satisfying user requirement. }



==> text/profiling_old.tex <==
\section{Adaptive Memory Profiling (2 pages)}
\label{sec:profiling}
x86 hardware does not support memory access counting at a per-page granularity. We track page accesses by utilizing PTE reserved bits and PTE table scan, similar to existing work~\cite{} for page management for HM. \textcolor{red}{(Jie: add more details on this method.)}


\textcolor{dong}{Scanning and setting access bits to track page accesses for large memory is expensive. For example, scanning a five-level page table for 1.5 TB memory in an Optane-based platform using one thread (see Table~\ref{tab:hardware}) takes xxxx--xxxx seconds.  %Setting access bits for xxxxx pages in that platform with a page size of 2 MB takes xxxxx seconds. 
To avoid such a large overhead, it is natural to sample pages for profiling. We introduce an adaptive memory profiling method to sample pages and maximize profiling quality with a given profiling overhead. Figure~\ref{fig:profile_workflow} shows the workflow of one profiling window in \name.}
%tracking a page access on our Optane-based platform (see Table~\ref{tab:hardware}) takes xxxxx microsecond, including a page table write (xxxx microsecond), the page table scan (xxxx microsecond), and xxxxxx (xxxx microsecond). Given a large memory system with a capacity of hundreds of GB to multiple TB, scanning the whole page table takes xxxxxx seconds. 

%\textcolor{jie2}{Memory access information is essential to guide memory management. However, tracking memory access from huge and complex applications in big memory system is non-trivial. There is a trade-off between profiling overhead and profiling accuracy. Prior works~\cite{pintool,simpoint} instrument load/store instruction in applications, which can get entire memory access trace. However, such frequent memory access monitoring incurs one or more orders of magnitude overhead. Sampling-based profiling method are explored to reduce profiling overhead. Hardware counter provided by x86 architecture such as PEBS (Precise Event Based Sampling) can record memory access events. Due to limited sampling frequency, hardware counter based profiling can not provide enough memory access information~\cite{}. Another widely used sampling-based profiling techniques rely on OS page management, which periodically scan PTE access bit~\cite{thermostat_asplos17, Hirofuchi:2016:RHV:2987550.2987570, memory_tiering, autonuma_balance, intel_mem_optimizer}.  However, without carefully select sampled pages, the profiling accuracy could dramatically decrease.}

%\textcolor{jie2}{We study the relation between profiling frequency and overhead of commonly used profiling methods, the result shows in table~\ref{tab:profiling_methods}. We profile memory access %for matrix-multiplication for a micro-benchmark with instrumentation-based profiling, hardware counter based sampling, and PTE access bit scanning. With same profiling overhead, PTE access bit scanning achieves highest page walk frequency. \name adopts PTE access bit scanning for efficient profiling. We further observe that the overhead of scanning PTE access bit is linear with the number of pages involving in profiling. Therefore, to ensure profiling overhead remains stable for all profiling window, \name profiles the same number of pages for all profiling window.}

%\input tables/profiling.tex

\begin{figure*}[tb]
\centering
\includegraphics[width=1.9\columnwidth]{figures/profile.pdf}
\caption{The overview of memory profiling in \name. 
\label{fig:profile_workflow}}
\end{figure*}



\subsection{\textcolor{jie}{Spatial Locality Oriented Sampling}}
%%%%\textcolor{jie}{introduce memory regions.}
\textcolor{jie2}{
\name profiles big memory system as a set of memory regions, where each memory region is contiguous virtual memory space. \name performs memory management based on memory region. The design of memory region is based on spatial locality. OSes maintain multi-level page table to record virtual address and physical address mapping. \name sets the default memory region size as the size of second last level page table entry corresponding memory space. \name \textit{adaptively} adjusts the size of memory regions based on the profiling results for upcoming profiling windows.}

\textcolor{jie2}{
To reduce profiling overhead, \name carefully selects and tracks representative pages access instead of all pages in a memory region to estimate the access information of whole memory region. 
For example, in profiling window $k$, there are $N_i(k)$ representative pages in memory region $i$. Each representative page goes through three consecutive PTE access bit scanning, which require checking the access bit status. The access frequency of each representative page is $A_{Ni}(m)$, where $m \in N_i(k)$. The profiler reports \textit{time-consecutive profiling results} of memory region $i$ as $A_i(k)$, which is the average number of memory access of all representative pages in memory region $i$. Please note that $A_i(k)$ indicates the hotness of memory region $i$. By comparing the access frequency of representative pages $A_{Ni}(m)$ in each memory region, \name makes memory region splitting decision. By comparing the memory access between contiguous memory region $A_i(k)$ and $A_{i+1}(k)$, \name makes memory region merging decision. 
%\name sets basic memory region size based on application memory consumption and user specified overhead. 
}


\subsection{\textcolor{jie}{Temporal Locality Oriented Profiling}}
\textcolor{jie2}{%%To reduce profiling overhead, \name carefully selects and tracks representative pages access instead of all pages in a memory region to estimate the access information of whole memory region. %To provide accurate profiling on each memory region, \name uses one or more representative pages in each memory region.
\name uses \textit{adaptive page sampling} to selective representative pages in each memory region.
\name decides the number of representative pages in each memory region by considering memory region access temporal locality. Representative pages selection in each memory region is random. 
Specifically, for memory regions which have similar access pattern across profiling windows, \name reduces the number of representative pages to track memory region accesses. To ensure the profiling accuracy of memory regions with different number of access among different profiling window, \name increases the number of representative pages in those memory regions. 
By considering the memory access history of the memory region $i$ and comparing $A_i(k)$ and $A_i(k-1)$, \name makes decision on increase/decrease the number of representative pages $N_i(k+1)$ in memory region $i$. Specifically, if $A_i(k) - A_i(k-1) > \tau$, \name increases the number of representative pages in memory region $i$.
}



%\textcolor{jie2}{We assume that there are $k_i$ representative pages in memory region $i$, where $k>0$. %The $k$ representative pages are randomly chosen in each profiling window. 
%The profiler in \name keeps memory access history for each memory region. We define $h_i(t)$ as the memory access history for memory region $i$ in profiling window $t$. \name decides the number of representative pages $k_i$ based on $h_i(t)$ and $h_i(t-1)$. Specifically, if $h_i(t-1) - h_i(t) > \tau$, \name increases the number of representative pages in memory region $i$. }

%%%The logic indicates that the tracing overhead and the accuracy of the traced output become greater as the number of regions increases and the time interval between sampling iterations decreases.
%%%thus allows users to control the upper bound of the tracing overhead and the quality of the output by setting the upper bound of the number of regions and the time interval. 
%%%histgram


\subsection{\textcolor{jie}{Profiling Quality Control}}
\textcolor{jie2}{The profiler in \name provides quality control by adaptive adjusting the size of memory regions. Multiple representative pages in each memory region might have different number of memory access be tracked. Based on the memory access tracking for each representative pages, \name merges or splits memory regions. Note that the total number of representative pages remains the same across profiling windows. 
}

\textcolor{jie2}{Memory region merging happens when the contiguous memory regions has similar access frequency. For memory region $i$ and its neighbor $i+1$, we compare the memory region access $A_i(k)$ and $A_{i+1}(k)$. For contiguous memory regions with same access pattern, \name merges them together to reduce the number of representative pages in those memory regions. }

\textcolor{jie2}{Memory region splitting happens when the multiple representative pages in the same memory region do not have similar memory access frequency. This indicates that the memory region is too coarse-grained. For those memory regions, \name splits it as two new memory regions with the same size. Specifically, for two representative pages $m$ and $n$ in memory region $i$, if $A_{Ni}(m) != A_{Ni}(n)$, \name splits memory region $i$ into two memory regions with equal size. Note that memory region splitting stops when the memory region is equal to the default memory region size.}

%\textcolor{jie}{split/merge memory region for profiling}


\subsection{\textcolor{jie}{Profiling Overhead control}}
\textcolor{jie2}{\name provides \textit{fine-grained profiling overhead control} by (1) choosing the size of memory region based on overhead estimation, (2)ensuring the total number of pages involves in PTE access bit scanning remain the same across profiling windows, and (3) adaptively pause PTE scanning at the end of profiling window. Such that \name ensures the profiling overhead satisfying user requirements.  }
%\textcolor{jie}{choose the granularity of  memory region for profiling}


\textcolor{red}{(discuss how to choose profiling overhead target)}



%\subsection{Discussion}
%\textcolor{jie2}{The profiler in \name provides quality control and overhead control, which aims to provide high quality memory region access tracing with limited profiling overhead. However, the profiling overhead could not be too small. \name increases the size of each memory region to reduce profiling overhead. Too small profiling overhead leads to carouse-grained profiling, such that the memory accesses of representative pages can not provide good indication on accesses in memory regions. }

%\textcolor{jie2}{Although region-based sampling method has been used in prior work~\cite{middleware19_profiling}, without correlation of time-consecutive profiling results, region-based sampling would impossible to provide useful memory migration hints, which are, in turn, useless in memory management. Meanwhile, time-consecutive profiling brings new challenges in profiling overhead control. }

